CompVPD: Iteratively Identifying Vulnerability Patches Based on Human Validation Results with a Precise Context

Applying security patches in open source software timely is critical for ensuring the security of downstream applications. However, it is challenging to apply these patches promptly because notifications of patches are often incomplete and delayed. To address this issue, existing approaches employ deep-learning (DL) models to identify additional vulnerability patches by determining whether a code commit addresses a vulnerability. Nonetheless, these approaches suffer from low accuracy due to the imprecise context provided for the patches. To provide precise context for patches, we propose a multi-granularity slicing algorithm and an adaptive-expanding algorithm to accurately identify code related to the patches. Additionally, the precise context enables to design an iterative identification framework, CompVPD, which utilizes the human validation results, and substantially improve the effectiveness. We empirically compare CompVPD with four state-of-the-art/practice (SOTA) approaches in identifying vulnerability patches. The results demonstrate that CompVPD improves the F1 score by 20% compared to the best scores of the SOTA approaches. Additionally, CompVPD contributes to security practice by helping identify 20 vulnerability patches and 18 fixes for high-risk bugs from 2,500 recent code commits in five highly popular open-source projects.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> analyzer/cases.tex <==
目前计划的新的文章思路：

我们观察到：现有的补丁识别工作对diff上下文考虑的不够全面：
●只考虑文本级别的上下文（修改行和上一行，下一行）
●只考虑函数内单个局部变量的上下文【只选择一个变量，然后保留一个函数内涉及到该变量上下文代码】

我们提出：应该扩充更多的上下文
●跨方法，甚至跨文件级别的上下文
●基于各种级别的代码关联，数据流、控制流

挑战：
●现有的模型输入window size有限（常见1k-2k），不可能全部装进去，即使装进去了对GPU资源（尤其是显存）的开销也较大

解决方案：基于预筛（去掉非java文件，测试文件）+切片的方式来扩充一个程序的diff的上下文：
●先切片，去掉和修改行对应代码无数据/控制以来的代码，函数调用；对没有修改但被调用的函数保留签名和docstring
●动态保留修改行的上下文，使其尽可能完整

- 向上：所有起点在行x里的，希望x尽可能小
- 向上：三行内保留有dependency or x层级变小
- 向上：保留注释的docString
（修一下def-use的问题）

实验：
关于扩充上下文之后的diff，我们通过deep-learning models，包括大模型来学习其特征：
●现有的deep-learning models AUC = 0.80&0.81 （baselines）
●（将切片后的特征图直接embedding后训练）AUC = 0.91
●基于开源大模型fine-tune后，AUC = 0.96，F1=0.7 （考虑到AUC可能已经不合适了）【我们的工作】
○观察到截断的非常严重，例如1k的window size，但平均一个diff有3k个tokens
●基于开源大模型fine-tune后+扩充的上下文，结果TBD
Ablation Study：
●不同的windows size（对应更多的上下文），是否对结果有影响
●我们的预筛+切片的思路方法在上下文总量不变的情况下，可以减少多少的输入规模
计算资源开销：时间+显存（可用性）
我们的方法在新的commit上扫描（比如2023年的），能扫出多少隐匿补丁（旧的结果是扫描了28个，15个被确认为隐匿补丁，其中10个是已经被官方承认的）

一个motivating example：
                 (inputFilters[Constants.CHUNKED_FILTER]);
             contentDelimitation = true;
         } else {
-            for (int i = 2; i < inputFilters.length; i++) {
+            for (int i = pluggableFilterIndex; i < inputFilters.length; i++) {
                 if (inputFilters[i].getEncodingName()
                     .().equals(encodingName)) {
                getInputBuffer().addActiveFilter(inputFilters[i]);


完整的上下文可能是：
 protected boolean addInputFilter(InputFilter[] inputFilters,
                                     String encodingName) {
        if (encodingName.equals("identity")) {
            // Skip
        } else if (encodingName.equals("chunked")) {
            getInputBuffer().addActiveFilter
                (inputFilters[Constants.CHUNKED_FILTER]);
            contentDelimitation = true;
        } else {
            for (int i = 2; i < inputFilters.length; i++) {
            for (int i = pluggableFilterIndex; i < inputFilters.length; i++) {
                if (inputFilters[i].getEncodingName()
                    .().equals(encodingName)) {
            getInputBuffer().addActiveFilter(inputFilters[i]);
                    return true;
                }
            }
            return false;
        }
        return true;
    }


   


最好变为：
protected boolean addInputFilter(InputFilter[] inputFilters,
                                     String encodingName) {
        if (encodingName.equals("identity")) {
        } else if (encodingName.equals("chunked")) {
        } else {
-            for (int i = 2; i < inputFilters.length; i++) {
+            for (int i = pluggableFilterIndex; i < inputFilters.length; i++) {
                if (inputFilters[i].getEncodingName()
                    .().equals(encodingName)) {
               getInputBuffer().addActiveFilter(inputFilters[i]);
                    return true;
                }
            }
            return false;
        }
    }

    

或者：
   protected boolean addInputFilter(InputFilter[] inputFilters,
                                     String encodingName) {
-            for (int i = 2; i < inputFilters.length; i++) {
+            for (int i = pluggableFilterIndex; i < inputFilters.length; i++) {
                if (inputFilters[i].getEncodingName()
                    .toString().equals(encodingName)) {
                    getInputBuffer().addActiveFilter(inputFilters[i]);
                    return true;
                }
            }
    }






positive generate:

real	0m9.527s
user	6m29.380s
sys	0m29.827s

negative generate:
real	17m43.929s
user	500m9.020s
sys	10m31.737s

real	17m43.575s
user	499m7.143s
sys	9m34.932s

增加一个迭代加深的算法
自适应调整长度




java.lang.IndexOutOfBoundsException: Index -1 out of bounds for length 0
	at java.base/jdk.internal.util.Preconditions.outOfBounds(Preconditions.java:64)
	at java.base/jdk.internal.util.Preconditions.outOfBoundsCheckIndex(Preconditions.java:70)
	at java.base/jdk.internal.util.Preconditions.checkIndex(Preconditions.java:248)
	at java.base/java.util.Objects.checkIndex(Objects.java:372)
	at java.base/java.util.ArrayList.get(ArrayList.java:459)
	at visitors.STMTVisitor.visit(STMTVisitor.java:110)
	at org.eclipse.jdt.core.dom.ContinueStatement.accept0(ContinueStatement.java:138)
	at org.eclipse.jdt.core.dom.ASTNode.accept(ASTNode.java:2711)
	at org.eclipse.jdt.core.dom.ASTNode.acceptChildren(ASTNode.java:2782)
	at org.eclipse.jdt.core.dom.Block.accept0(Block.java:137)
	at org.eclipse.jdt.core.dom.ASTNode.accept(ASTNode.java:2711)
	at org.eclipse.jdt.core.dom.ASTNode.acceptChild(ASTNode.java:2759)
	at org.eclipse.jdt.core.dom.IfStatement.accept0(IfStatement.java:191)
	at org.eclipse.jdt.core.dom.ASTNode.accept(ASTNode.java:2711)
	at org.eclipse.jdt.core.dom.ASTNode.acceptChildren(ASTNode.java:2782)
	at org.eclipse.jdt.core.dom.Block.accept0(Block.java:137)
	at org.eclipse.jdt.core.dom.ASTNode.accept(ASTNode.java:2711)
	at org.eclipse.jdt.core.dom.ASTNode.acceptChild(ASTNode.java:2759)
	at org.eclipse.jdt.core.dom.IfStatement.accept0(IfStatement.java:192)
	at org.eclipse.jdt.core.dom.ASTNode.accept(ASTNode.java:2711)
	at org.eclipse.jdt.core.dom.ASTNode.acceptChildren(ASTNode.java:2782)
	at org.eclipse.jdt.core.dom.Block.accept0(Block.java:137)
	at org.eclipse.jdt.core.dom.ASTNode.accept(ASTNode.java:2711)
	at org.eclipse.jdt.core.dom.ASTNode.acceptChild(ASTNode.java:2759)
	at org.eclipse.jdt.core.dom.Initializer.accept0(Initializer.java:252)
	at org.eclipse.jdt.core.dom.ASTNode.accept(ASTNode.java:2711)


==> analyzer/dataset_detail.tex <==
https://github.com/blynkkk/blynk-server (not found)
https://github.com/javaserverfaces/mojarra (archived)
https://github.com/angelozerr/lsp4xml (name changed to https://github.com/eclipse/lemminx)
https://github.com/droolsjbpm/jbpm-designer (name changed to https://github.com/kiegroup/jbpm-designer)
https://github.com/wuyouzhuguli/FEBS-Shiro (not found)
https://github.com/dotCMS/dotCMS (changed to https://github.com/dotCMS/core)

1474 vulnerability fixes -> 1355 vulnerabilities (completely duplicated, (119))

{'test_loss': 0.25562360882759094, 'test_auc': 0.9308628503801029, 'test_f1_best': 0.3166023166023166, 'test_f1_threshold': 0.98291015625, 'test_mcc_best': 0.3145192556216451, 'test_mcc_threshold': 0.98291015625, 'test_num_samples': 71381, 'test_runtime': 7192.1357, 'test_samples_per_second': 9.925, 'test_steps_per_second': 0.052}


real    19m8.167s
user    538m41.192s
sys     8m51.775s

real    0m11.248s
user    8m3.337s
sys     0m25.894s

real    15m14.420s
user    418m53.073s
sys     10m41.195s

real    0m10.498s
user    6m42.109s
sys     0m34.867s

==> analyzer/miss_repo.tex <==
miss train repo
['https://github.com/kawasima/struts1-forever', GHTML proj, Java < 21\%, more than 5 years without commit
 'https://github.com/dotCMS/dotCMS', name changed to dotCMS/core             
 'https://github.com/javaserverfaces/mojarra', name changed to eclipse-ee4j/mojarra
 'https://github.com/dom4j/dom4j', normal
 'https://github.com/JabRef/jabref', normal
 'https://github.com/angelozerr/lsp4xml', name changed to eclipse/lemminx
 'https://github.com/OWASP/json-sanitizer', normal
 'https://github.com/checkstyle/checkstyle', normal
 'https://github.com/Wechat-Group/weixin-java-tools', name changed to https://github.com/Wechat-Group/WxJava
 'https://github.com/codehaus-plexus/plexus-archiver',
 'https://github.com/spring-projects/spring-data-jpa', normal
 'https://github.com/apache/cordova-plugin-file-transfer', js proj (more than 57\%)
 'https://github.com/naver/ngrinder', normal
 'https://github.com/apache/spark', scala proj, normal
 'https://github.com/blynkkk/blynk-server', not found
 'https://github.com/bigbluebutton/bigbluebutton'] javascript (more than 56\%)

miss test repo
 ['https://github.com/PebbleTemplates/pebble', normal
 'https://github.com/wuyouzhuguli/FEBS-Shiro',
 'https://github.com/facebook/fbthrift', C++ proj, more than 53\% java less than 11\%, rank 3
 'https://github.com/akka/akka-http', (scala proj), normal
 'https://github.com/hawtio/hawtio', normal
 'https://github.com/droolsjbpm/jbpm-designer', name changed to kiegroup/jbpm-designer
 'https://github.com/nahsra/antisamy', java less than 20\% rank 3
 'https://github.com/manolo/gwtupload'], more than three years out of commit



current:

[
blynkkk/blynk-server  & not found                              
wuyouzhuguli/FEBS-Shiro    & not found                         
angelozerr/lsp4xml       & name changed to eclipse/lemminx     
droolsjbpm/jbpm-designer & name changed to kiegroup/jbpm-designer
dotCMS/dotCMS        & name changed to dotCMS/core             
javaserverfaces/mojarra       & name changed to eclipse-ee4j/mojarra    
]




miss train repo

['https://github.com/kawasima/struts1-forever',
 'https://github.com/dotCMS/dotCMS',
 'https://github.com/javaserverfaces/mojarra',
 'https://github.com/dom4j/dom4j',
 'https://github.com/JabRef/jabref',
 'https://github.com/angelozerr/lsp4xml',
 'https://github.com/OWASP/json-sanitizer',
 'https://github.com/checkstyle/checkstyle',
 'https://github.com/Wechat-Group/weixin-java-tools',
 'https://github.com/codehaus-plexus/plexus-archiver',
 'https://github.com/spring-projects/spring-data-jpa',
 'https://github.com/apache/cordova-plugin-file-transfer',
 'https://github.com/naver/ngrinder',
 'https://github.com/apache/spark',
 'https://github.com/blynkkk/blynk-server',
 'https://github.com/bigbluebutton/bigbluebutton']



miss test repo
['https://github.com/PebbleTemplates/pebble',
 'https://github.com/wuyouzhuguli/FEBS-Shiro',
 'https://github.com/facebook/fbthrift',
 'https://github.com/akka/akka-http',
 'https://github.com/hawtio/hawtio',
 'https://github.com/droolsjbpm/jbpm-designer',
 'https://github.com/nahsra/antisamy',
 'https://github.com/manolo/gwtupload']

==> analyzer/refine.tex <==
CompVPD

为什么不考虑context就会带来问题：xxx
Context的定义是什么，没有这个context就会导致什么问题：
要具体讲清楚context是什么

传统的slicing解决不了
Complete的定义：基于代码块去做定义
举一个例子说明：不完整会xxx

《例子》：这个信息要加上后面xxx信息才能一起做判断



要把这个例子讲透
比如同一个语句，

我加了context之后，引入了什么新的困难
这个事情要说出来：《基于一个预训练的模型微调》

比如这应该是一个局部化的slicing，那我们应该xxx，怎么选context width合适，（现有的方法都是固定长度的xxx）


max context width的定义

没有一个trade-off，单纯就说它装不下就行

1.定义清楚
2.现有方法的局限要讲透







==> tab/ase23_comments.tex <==
ASE2023 Paper #108 Reviews and Comments
===========================================================================
Paper #108 Identifying Vulnerability Patches with Graph Representation of
Multiple Changed Functions


Review #108A
===========================================================================

Overall merit
-------------
2. Weak reject

Paper summary
-------------
In this paper, authors provide a new tool called MultiVP – which is claimed to be the first approach to identify vulnerability patches with multiple changed functions by utilizing graph neural networks.
The research has been done on a newly constructed vulnerability patch dataset (VulPatch), as well as the existing one (VulFixJava), and shows promising results.

Strengths
---------
- Focus on practitioners, partially using the dataset from the industry, is a huge plus.
- The results seem to be better than the baselines.

Weaknesses
----------
Weaknesses:
- The claim that the proposed tool can also work with C/C++ should be verified (or removed?)

【可以不去强调c++这个事情，反正我们也没做】

- Using a weak performance measure (see the detailed weaknesses below) and calling the comparison comprehensive can lead to false conclusions

【这个审稿人推荐了MCC，应该是同一个人，这次我们可以加上F1和MCC】

- RQ3 is superficially reported vide "Due to the space limit, the results can be found on our anonymous website [38]." Thus either report it properly or remove it.
【把这个RQ去掉，RQ3: How much benefit can security practice gain from our approach?】
【文章里还有个地方把RQ3的标题写成了RQ2的，更加misleading】
- The description of Threats To Validity seems to be limited.
【重写一下Threats To Validity，external还是写数据集可能标注的有问题，internal就写DL models的parameters，construction加上metric】
- The paper does not provide the links to the tool, so reproducibility and verifiability are nonexistent. 
- No reproduction package was provided.
【没有开源，这个最多把数据放出去（比如夏鑫他们的数据集）】

Detailed weaknesses:
- "Metrics: We evaluate the effectiveness of patch identification models by the area under the curve (AUC) [16], which is used to measure a model’s prediction performance for all discrimination thresholds ranging from 0 to 1. AUC is defined as the area under the receiver operating characteristic (ROC) curve, and a ROC curve plots this model’s true-positive rates against its false-positive rates at various discrimination thresholds. When compared with other threshold-dependent metrics, such as precision, recall, and F1, AUC is robust in imbalanced datasets (i.e., the number of positive samples is significantly less than that of negative samples) because it does not depend on any specific discrimination threshold [37]." - I recommend to take into account that "The Matthews correlation coefficient (MCC) should replace the ROC AUC as the standard metric for assessing binary classification", see D. Chicco and G. Jurman, “The Matthews correlation coefficient (MCC) should replace the ROC AUC as the standard metric for assessing binary classification,” BioData Mining, vol. 16, no. 1, p. 4, 2023.
【同上，这个审稿人推荐了MCC，应该是同一个人，这次我们可以加上F1和MCC】

- "RQ3: To what extent can our graph reduction algorithms improve MultiVP’s efficiency?"  - RQ3 is, in fact, superficially reported vide "Due to the space limit, the results can be found on our anonymous website [38]." and thus either report it properly or remove.
【这个RQ要改一下，本来说的是我们拿这个工具扫出来的结果，但我就放了一个list在网站上；改成：我们扫描了xxx个commit，扫出来xxx个，xxx个经人工确认是隐匿补丁，文章里放两个case study（比如taotao之前看的二十几个）】
- "Identifying vulnerability patches of other programming languages: MultiVP has enough generalization ability to identify vulnerability patches of other programming languages. Take C/C++ as an example, it can identify C/C++ vulnerability patches after training on a set of C/C++ vulnerability patches, whose CPGs can be generated based on a C/C++ parser (e.g., CDT [7]). We implement and evaluate MultiVP on Java vulnerability patches mainly because Java is one of the most widely used programming languages, especially for open- source repositories [49]." - the claim about the generalization ability of MultiVP is not supported in any way in the paper and, thus, should not be raised in the Discussion section.
【能否在C/C++上通用，当然是可以的，但我们既然没做这个实验，就不要提这个事情了 “should not be raised in the Discussion section”】
- "For each vulnerability, we randomly require two senior software engineers to independently label and validate the affected libraries of this vulnerability." - It is unclear how possible conflicts were resolved. There are also too few details about "senior software engineers". 
【数据标注，还是老问题，两个解决方案：（1）就说我们自己的数据集主要是基于GitHub的（图模型数据的正样本版本也比较老，后续标注的也不在里面），然后放出去；（2）只保留夏鑫的数据上跑出来的结果】
- Some of the statements are not supported by, e.g., a systematic review or a reference to a systematic review:
-- "we are the first approach to identify vulnerability patches with multiple changed functions by graph neural networks.", "To address the limitation of low accuracy faced by the existing approaches, we design MultiVP, the first approach to identify vulnerability patches with multiple changed functions..."
-- " Other approaches do not consider algorithms (1) and (2), and only two of them [51], [45] use algorithm (3) for graph reduction."
-- "In this paper, we have presented MultiVP, the first approach to identify vulnerability patches with multiple changed functions by graph neural networks."
【加一个systematic review，整理一下现有的方法，他们基于xxx，用到了xxx】

- Minor issue:
-- "CoderBert [11]" -> CodeBert [11]

Comments for authors
--------------------
In this paper, the authors provide a new tool called MultiVP – which is claimed to be the first approach to identify vulnerability patches with multiple changed functions by utilizing graph neural networks.
The research has been done on a newly constructed vulnerability patch dataset and the existing one, and shows promising results. Shown focus on practitioners' perspectives and partially using the dataset from the industry is a huge plus. However, the paper does not provide the links to the tool, so reproducibility and verifiability are nonexistent. 
Also, the claim that the proposed tool can also work with C/C++ should be verified (or removed?). Using only one performance measure (and an imperfect one) and calling the comparison comprehensive can lead to false conclusions (see detailed weaknesses and the paper by Chicco and Jurman 2023). Lastly, Threats To Validity could be expanded, at least by the abovementioned issues.

Significance: High – vulnerability detection is a very important field of study from both, academic and industry perspectives.
Novelty: High – authors propose a new tool that may outperform the current state-of-the-art methods (but it needs to be checked using MCC).
Soundness: Average/Low - paper’s contributions and innovations partly address the designed research questions and are supported by partly adequate research methods (see my comments about RQ3 and the performance measure used by the authors).
Verifiability: Low - The paper does not provide the links to the tool, and there is no reproduction package provided, so reproducibility and verifiability are low.
Transparency: Low - Authors offer adequate information to understand how the proposed approach works and how data was obtained, analyzed, and interpreted; however, they do not provide the data and the developed tool itself.
Presentation High - the paper is very well written and formatted.



Review #108B
===========================================================================

Overall merit
-------------
2. Weak reject

Paper summary
-------------
This paper introduces MultiVP, an approach to detect whether or not a given commit fixes a vulnerability in a java code base.
MultiVP leverages code property graphs (CPG) in order to capture relevant information about code changes.
The authors also present three methods to reduce the size of CPGs, and show them to enable a massive speedup in training time, with only a moderate loss in accuracy.
A novel dataset of vulnerability patches in introduced, though not yet released.

Strengths
---------
- Comprehensive approach
- Contributions to several major challenges in the field

Weaknesses
----------
- A bit hard to follow at times
【文章结构需要重构一下】
- Verifiability and impact limited by the lack of released implementation
【开源的问题】

Comments for authors
--------------------
The topic addressed is important, and is an active field of research.

This approach proposes significant novel contributions in:
- What information to capture, with custom CPGs;
- What information to discard/reduce, to speed up the training time, which can otherwise be a bottleneck;
- How to embed the CPGs.

One potential improvement for this paper would be to better explain what parts of the CPGs used are designed specifically for this work, and what parts are consistent with prior work.

【CPG里哪些部分比较重要，不能删除，哪些部分不重要，可以删除，删掉哪些部分能提高效率；这个可能需要一些case studies；如果我们后续不强调CPG，那这个就不重要了】

This paper would also benefit from a complete proofread, to fix several weird and/or invalid sentences, though it does not really hinder the comprehension.

- The RQ3 (p9) does not match the RQ3 presented at the beginning of section 4.
- And RQ3 would also deserve more space. At the very least, the authors should clarify whether the 17 "Java vulnerabilities identified" are actually vulnerabilities, or are vulnerability patches. 
- Either way, having an indication of the true positive ratio (i.e., 17 out of how many?) would be interesting.
【同上，RQ3需要好好重写一遍】


# Typos:

p3 "MultiVP first extract" -> extracts

p3 "MultiVP mark" -> marks

p3: "even if some of them can be called actually (unreachable edges)"  did you mean 'that canNOT be called'?

p6, definition of V: "D1, D2" -> D_1, D_2

p6 "a irrelevant" -> an

p6 "and the code commit" -> and one code commit

p7 "not open-source available" -> not available under an open-source licence (or just: not open-source)

p7 "We use the CPU of Xeon[...]@2.3GHz" -> We use one Xeon[...]@2.3GHz CPU, which [...]

p7 "We use 8 GPUs of Tesla V100 PCIe with 32GB of memory" -> We use 8 Tesla V100 PCIe GPUs with 32GB of memory for model training

p9 "the improvements of MultiVP mainly credits to our" -> the improvements of MultiVP are mainly due to our

Table 1: Boxplots wouldn't take much more space, but would be easier to read.
【修一下这些typo就行】


Review #108C
===========================================================================

Overall merit
-------------
1. Reject

Paper summary
-------------
The existing deep-learning assist method to determine if a code commit is a vulnerability patch, suffering from low accuracy. To overcome the low accuracy, this paper proposes to use CPG to represent code commits with three Graph reduction methods.

Strengths
---------
- Target an important problem

Weaknesses
----------
- Lack of evaluation on the effectiveness of the graph representation of multiple changed functions
【标题/intro里强调了multiple changed functions，需要evaluation对应上；可能不必强调这个事情】
- Limited technical contributions
- Problematic or unclear motivation
【这俩是挺根本的问题，文章的整体思路要改一下】
- Incorrect claims about the related work
【修改关于VulFixMiner的描述，他们至少是file-level的，只是做的不好（而不是说他们是function-level）】
- Source code is not available
【代码估计没办法，我们最多把可以公开的数据开源】

Comments for authors
--------------------
This paper designs CPG to represent the code commits with three graph reduction algorithms, using the GCN model to learn the dependencies of vulnerability patches. This is a straightforward method, however, I have the following concerns.

- One of my main concerns is the motivation and some claims about the existing work. The authors claim "These existing approaches take only one changed function as their input, ignoring multiple changed functions of a code commit as input", however, as described in the paper of VulFixMiner, it extracts file-level code changes, i.e., including multiple function changes. Therefore, the motivation seems problematic and unclear, and the contribution is limited. The differences between the existing work and the proposed method should be appropriately highlighted.
【加一个systematic review，整理一下现有的方法，尤其不要强调VulFixMiner不是function-level的，就说它是file-level实现的repo-level】

- How to determine which changed commits are related to vulnerability patches, and how to verify it.
【这个我们可以描述一下，人工验证/标注的思路】

- In the dataset, if there is only one changed function, how to label it and handle it? Did such cases be handled currently?
【也是数据集标注的问题，我们并不区分这个；最好也别强调multi-function】

- The evaluation section in this paper shows better efficiency compared to MultiVP with baseline, and the new dataset. But the effectiveness and efficiency of the graph representation of multiple changed functions aren't presented.
【是否区分multiple changed functions，我们实验里也许可以看一下，修改函数/文件（=1） & （>1）是否有区别，不需要额外训练】

- RQ3 does not convey any useful information, at least showing some primary or simplified result.
【同上，RQ3需要好好重写一遍】


Review #108D
===========================================================================

Metareview
----------
As reviewers, we’ve found the following strengths of this paper:

- Target an important problem.
- Focus on practitioners, partially using the dataset from the industry, is a huge plus.
- The results seem to be better than the baselines.
- Potential contributions to major challenges in the field.
However, we’ve also found the following weaknesses:

- Incorrect claims and problematic or unclear motivation (e.g., about the related work which makes motivation problematic and unclear and thus contribution limited; the claim that the proposed tool can also work with C/C++ should be verified or removed).
【motivation】

- Lack of evaluation on the effectiveness of the graph representation of multiple changed functions.
【不强调multiple changed functions了】
- Using only one (and an imperfect one) performance measure (see Chicco and Jurman 2023) and calling the comparison comprehensive can lead to false conclusions.
【关于MCC metrics，这个加上就行】
- RQ3 is superficially reported (see "Due to the space limit, the results can be found on our anonymous website [38].”). Thus either report it properly or remove it.
【RQ3】
- Non-available source code, which limits verifiability, transparency and impact of the paper.
【开源】

All reviewers agreed that the paper is not ready to be accepted now, thus recommending rejection, but we all hope that the spotted weaknesses will help the authors to improve the paper.

Recommendation
--------------
C. Reject










解决方案：
- 做一个empirical study：基于代码特征表示的补丁识别【包括序列模型（xiaxin），图模型，序列模型+大模型，图切片+大模型】
- 现有工作拆成两个【图模型按照之前的修改意见修，然后投一个industrial之类的】【大模型的思路：基于图切片+大模型的补丁识别】

现象：现有的模型无法处理过长的输入【要么只保留一部分；要么按照文件/函数级别分开处理】
我们的解决方案：基于图的剪枝 & 剪枝之后的大模型？

（问题：怎么把大模型和图模型结合起来）

论点：我们提出应该通过基于切片+排序的方式来表示一个程序的diff：
- 切片：去掉非java文件，测试文件，xxx；diff保留修改行附近多少行
- 排序：剩下的java文件里保留哪些（按优先级排序，然后只保留靠前的）；压缩


1.  cross project & mix project的数据集（数据集，2023-09-01）
2.  模型：CodeBert -> PangGuCoder -> StartCoder
3. Context：原始diff -> 切上下文
4.  window size 不够，如何解决？
	切片算法优化
              使用级联增加 window size

试验（code diff + commit msg）：
   1. cross project StarCoder（2K） + 切片扩充的效果 【潜涛涛】   【2023-09-08】
   1. StarCoder (参数更大，window 2K) 不切片的效果：cross and mix 【潜涛涛】   【2023-09-15】
  2.  CodeBert*2 【2023-09-03】【陈天宇】
    4. PanguCoder（window size 512 -> 1024）消融试验 比较 512 和 1K区别 *4【2023-09-08】【陈天宇】
  3*. 图模型 *2   【2023-09-18】【陈天宇】
  

==> tab/dataset_cmp.tex <==
repo	commit_id	cve_id	manually checked	ref website	
https://github.com/RadarCOVID/radar-covid-backend-dp3t-server	6d30c92cc8fcbde3ded7e9518853ef278080344d	CVE-2020-26230	NOT SURE		
https://github.com/FasterXML/jackson-databind	5f7c69bba07a7155adde130d9dee2e54a54f1fa5	CVE-2019-12814	NOT SURE	NVD is being modified	
https://github.com/cloudfoundry/uaa	2551072bb6a65592d316948e98c2819e12a29ba2		NOT SURE	Bouncy Castle Java library's vulnerability, this repo only use this lib	
https://github.com/apache/struts	f420f28466cb82915defc4e12466b298c275abaf		NOT SURE	Solves issue with vulnerable parameters	
https://github.com/RadarCOVID/radar-covid-backend-dp3t-server	6d30c92cc8fcbde3ded7e9518853ef278080344d	CVE-2020-26230	NOT SURE	duplicated	
https://github.com/spring-projects/spring-security-oauth	84d4efe1a89a6209799ad8e20fcfac8f24a18aa3		FALSE	it claims to fix a vulnerability, while it only add a judgement to return `equal` when two arraies are both null.	
https://github.com/rweather/noise-java	3b897f2d68d542ad0b538db2bf3a63790b5fe78a	CVE-2020-25021	FALSE	quite similar while NVD contain its real patch	
https://github.com/apache/hive	baaf082b1f3974a5f49c0cb7187ce9d2ab038e89		FALSE	marked as improvement, even not bug	unintentional  commit (daemon web UI vulnerabilities)
https://github.com/rweather/noise-java	dabedd0a110bf6b4ab103ba79a2df36db2b40289	CVE-2020-25021	FALSE	patch inproperly given in NVD	NVD - CVE-2020-25021 (nist.gov)
https://github.com/apache/commons-compress	654222e628097763ee6ca561ae77be5c06666173	CVE-2012-2098	FALSE	this commit only add lots of braces	
https://github.com/apache/tomcat	e28dd578fad90a6d5726ec34f3245c9f99d909a5	CVE-2014-0230	FALSE	seems negative samples	
https://github.com/rweather/noise-java	3b897f2d68d542ad0b538db2bf3a63790b5fe78a	CVE-2020-25021	FALSE	patch inproperly given in NVD	NVD - CVE-2020-25021 (nist.gov)
https://github.com/apache/hive	baaf082b1f3974a5f49c0cb7187ce9d2ab038e89		FALSE	duplicated	
https://github.com/rweather/noise-java	dabedd0a110bf6b4ab103ba79a2df36db2b40289	CVE-2020-25021	FALSE	patch given in NVD	NVD - CVE-2020-25021 (nist.gov)
https://github.com/netty/netty	e24e06bfcb8114270d46572cf96af49be76237b1				


==> tab/rq3.tex <==
repo_path	commit_id	commit_message	commit_time
https://github.com/jlangch/venice	c942c73136333bc493050910f171a48e6f575b23	"vuln-fix: Partial Path Traversal Vulnerability

This fixes a partial path traversal vulnerability.

Replaces `dir.getCanonicalPath().startsWith(parent.getCanonicalPath())`, which is vulnerable to partial path traversal attacks, with the more secure `dir.getCanonicalFile().toPath().startsWith(parent.getCanonicalFile().toPath())`.

To demonstrate this vulnerability, consider `""/usr/outnot"".startsWith(""/usr/out"")`.
The check is bypassed although `/outnot` is not under the `/out` directory.
It's important to understand that the terminating slash may be removed when using various `String` representations of the `File` object.
For example, on Linux, `println(new File(""/var""))` will print `/var`, but `println(new File(""/var"", ""/"")` will print `/var/`;
however, `println(new File(""/var"", ""/"").getCanonicalPath())` will print `/var`.

Weakness: CWE-22: Improper Limitation of a Pathname to a Restricted Directory ('Path Traversal')
Severity: Medium
CVSSS: 6.1
Detection: CodeQL & OpenRewrite (https://public.moderne.io/recipes/org.openrewrite.java.security.PartialPathTraversalVulnerability)

Reported-by: Jonathan Leitschuh <Jonathan.Leitschuh@gmail.com>
Signed-off-by: Jonathan Leitschuh <Jonathan.Leitschuh@gmail.com>

Bug-tracker: https://github.com/JLLeitschuh/security-research/issues/13

Co-authored-by: Moderne <team@moderne.io>"	2022/7/29 21:38
https://github.com/pgjdbc/pgjdbc	739e599d52ad80f8dcd6efedc6157859b1a9d637	"Merge pull request from GHSA-r38f-c4h4-hqq2

Fixes SQL generated in PgResultSet.refresh() to escape column identifiers so as to prevent SQL injection.

Previously, the column names for both key and data columns in the table were copied as-is into the generated
SQL. This allowed a malicious table with column names that include statement terminator to be parsed and
executed as multiple separate commands.

Also adds a new test class ResultSetRefreshTest to verify this change."	2022/8/2 0:46
https://github.com/srikanth-lingala/zip4j	5013235937636ba00bf3439374842a7588c86452	"vuln-fix: Partial Path Traversal Vulnerability (#466)

This fixes a partial path traversal vulnerability.

Replaces `dir.getCanonicalPath().startsWith(parent.getCanonicalPath())`, which is vulnerable to partial path traversal attacks, with the more secure `dir.getCanonicalFile().toPath().startsWith(parent.getCanonicalFile().toPath())`.

To demonstrate this vulnerability, consider `""/usr/outnot"".startsWith(""/usr/out"")`.
The check is bypassed although `/outnot` is not under the `/out` directory.
It's important to understand that the terminating slash may be removed when using various `String` representations of the `File` object.
For example, on Linux, `println(new File(""/var""))` will print `/var`, but `println(new File(""/var"", ""/"")` will print `/var/`;
however, `println(new File(""/var"", ""/"").getCanonicalPath())` will print `/var`.

Weakness: CWE-22: Improper Limitation of a Pathname to a Restricted Directory ('Path Traversal')
Severity: Medium
CVSSS: 6.1
Detection: CodeQL & OpenRewrite (https://public.moderne.io/recipes/org.openrewrite.java.security.PartialPathTraversalVulnerability)

Reported-by: Jonathan Leitschuh <Jonathan.Leitschuh@gmail.com>
Signed-off-by: Jonathan Leitschuh <Jonathan.Leitschuh@gmail.com>

Bug-tracker: https://github.com/JLLeitschuh/security-research/issues/13

Co-authored-by: Moderne <team@moderne.io>

Co-authored-by: Moderne <team@moderne.io>"	2022/9/8 21:34
https://github.com/apache/tomcat	c64d496dda1560b5df113be55fbfaefec349b50f	"Fix BZ 66471 - JSessionId secure attribute missing with RemoteIpFilter and X-Forwarded-Proto set to https

https://bz.apache.org/bugzilla/show_bug.cgi?id=66471
"	2023/2/9 22:48
https://github.com/DSpace/DSpace	56e76049185bbd87c994128a9d77735ad7af0199	"[DS-4131] Better path handling in ItemImport zips
"	2022/7/26 12:18
https://github.com/apache/fineract	7d2121d8cd50f962f8b423fbf7cd7cbb6c17ccd4	"FINERACT-1835: Backported fix of `Wrong audit time is set for datatables`
"	2022/12/15 19:59
https://github.com/GoogleContainerTools/jib	67fa40bc2c484da0546333914ea07a89fe44eaaf	"Check if file exists when executable path is passed in through jib dockerClient.executable (#3744)

* Check if file exists when executable path is passed in through jib.dockerClient.executable"	2022/8/26 4:23
https://github.com/spring-projects/spring-session	c98a7be0e2ced7f795018f05397dca4bd5ca8212	"Remove System.out.println

Closes gh-2215
"	2022/12/1 21:17
https://github.com/xwiki/xwiki-platform	3193716e5fbbc3e06d54d764dfa5e7c2d5e1ed63	"XWIKI-20312: Improved Live Data macro data parameter computation
"	2022/11/17 21:19
https://github.com/xwiki/xwiki-platform	df596f15368342236f8899ca122af8f3df0fe2e8	"XWIKI-20280: Improved link display for FlamingoThemesCode.WebHomeSheet
"	2022/11/22 23:59
https://github.com/xwiki/xwiki-platform	49fdfd633ddfa346c522d2fe71754dc72c9496ca	"XWIKI-20291: Improved translations of logging administration
"	2022/10/28 21:35
https://github.com/jenkinsci/script-security-plugin	806af0ad8c12d33757f6d97b41b3905e4237e641	"Fields declared in java.lang.Class must not shadow static fields when setting attributes
"	2022/10/20 22:48
https://github.com/jenkinsci/script-security-plugin	c1f529581ddd145d109c12dcb187db65af97e911	"Merge pull request #465 from jglick/HasherScriptApprovalTest

Never try to treat `URL.path` as a file path"	2022/11/16 3:28
https://github.com/cbeust/testng	9150736cd2c123a6a3b60e6193630859f9f0422b	"Merge pull request #2806 from BulkSecurityGeneratorProjectV2/fix/JLL/zip-slip-vulnerability

[SECURITY] Fix Zip Slip Vulnerability
"	2022/10/5 1:14
https://github.com/ManyDesigns/Portofino	94653cb357806c9cf24d8d294e6afea33f8f0775	"vuln-fix: Temporary Directory Hijacking or Information Disclosure



This fixes either Temporary Directory Hijacking, or Temporary Directory Local Information Disclosure.

Weakness: CWE-379: Creation of Temporary File in Directory with Insecure Permissions
Severity: High
CVSSS: 7.3
Detection: CodeQL & OpenRewrite (https://public.moderne.io/recipes/org.openrewrite.java.security.UseFilesCreateTempDirectory)

Reported-by: Jonathan Leitschuh <Jonathan.Leitschuh@gmail.com>
Signed-off-by: Jonathan Leitschuh <Jonathan.Leitschuh@gmail.com>

Bug-tracker: https://github.com/JLLeitschuh/security-research/issues/10


Co-authored-by: Moderne <team@moderne.io>"	2022/10/4 8:22
https://github.com/aws-amplify/aws-sdk-android	c3e6d69422e1f0c80fe53f2d757b8df97619af2b	"fix(core): added fix for xml parser (#3100)

* added fix for xml parser vulnerability

* added fix for xml parser vulnerability

Co-authored-by: Banji Jolaoso <banjij@amazon.com>"	2022/12/5 15:56
https://github.com/xwiki/xwiki-platform	d9e947559077e947315bf700c5703dfc7dd8a8d7	"XWIKI-16285: Error when accessing deleted document
"	2022/11/2 22:34


==> tab/rq_backup.tex <==
(61, 66)
(76, 86)
(99, 114)
(112, 135)
(120, 151)


({'recall': 0.3252032520325203, 'threshold': 0.9989652633666992}, 80.0)


==> tab/time_log.tex <==
(PyTorch-2.0.0) root@34229c669655:/data/chentianyu/silentVuln/LLM/starcoder/scripts# ./run_exp_3.sh 
[2023-09-06 20:11:47,013] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-06 20:11:49,856] [WARNING] [runner.py:201:fetch_hostfile] Unable to find hostfile, will proceed with training with local resources only.
[2023-09-06 20:11:49,987] [INFO] [runner.py:567:main] cmd = /home/ma-user/anaconda3/envs/PyTorch-2.0.0/bin/python -u -m deepspeed.launcher.launch --world_info=eyJsb2NhbGhvc3QiOiBbMCwgMSwgMiwgM119 --master_addr=127.0.0.1 --master_port=29500 --enable_each_rank_log=None /data/chentianyu/silentVuln/LLM/starcoder/finetune_with_trainer.py --model_path /data/qiantaotao/base_models/starcoderbase --deepspeed /data/chentianyu/silentVuln/LLM/starcoder/ds_config_zero_3.json --output_dir /efs_data/chentianyu/VulFixMiner/checkpoints/exp_3 --per_device_eval_batch_size 48 --per_device_train_batch_size 16 --num_train_epochs 10 --logging_steps 10 --gradient_checkpointing true --remove_unused_columns false --fp16 true --load_best_model_at_end true --include_inputs_for_metrics true --data_seed 42 --learning_rate 1e-4 --weight_decay 0.05 --save_strategy epoch --evaluation_strategy epoch --optim adamw_torch --data_dir /data/chentianyu/VulFixMiner/v1_dataset/v1_context --data_split_path /data/chentianyu/VulFixMiner/v2_dataset/cross_split.json --datasets_cache_dir /data/chentianyu/VulFixMiner/cache --max_seq_length 1024 --neg_ratio 10 --test_only false --diff_hunk_col commit_diff --r 16 --lora_alpha 32 --lora_dropout 0.05
[2023-09-06 20:11:51,865] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-06 20:11:53,650] [INFO] [launch.py:138:main] 0 NCCL_VERSION=2.13.4-1
[2023-09-06 20:11:53,650] [INFO] [launch.py:145:main] WORLD INFO DICT: {'localhost': [0, 1, 2, 3]}
[2023-09-06 20:11:53,650] [INFO] [launch.py:151:main] nnodes=1, num_local_procs=4, node_rank=0
[2023-09-06 20:11:53,650] [INFO] [launch.py:162:main] global_rank_mapping=defaultdict(<class 'list'>, {'localhost': [0, 1, 2, 3]})
[2023-09-06 20:11:53,650] [INFO] [launch.py:163:main] dist_world_size=4
[2023-09-06 20:11:53,650] [INFO] [launch.py:165:main] Setting CUDA_VISIBLE_DEVICES=0,1,2,3
[2023-09-06 20:11:57,084] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-06 20:11:57,121] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-06 20:11:57,174] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-06 20:11:57,186] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-06 20:12:00,944] [INFO] [comm.py:631:init_distributed] cdb=None
[2023-09-06 20:12:00,944] [INFO] [comm.py:631:init_distributed] cdb=None
[2023-09-06 20:12:00,944] [INFO] [comm.py:662:init_distributed] Initializing TorchBackend in DeepSpeed with backend nccl
[2023-09-06 20:12:01,054] [INFO] [comm.py:631:init_distributed] cdb=None
[2023-09-06 20:12:01,055] [INFO] [comm.py:631:init_distributed] cdb=None
2023-09-06 20:12:01-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 3
2023-09-06 20:12:01-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 2
2023-09-06 20:12:01-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 1
2023-09-06 20:12:01-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 0
2023-09-06 20:12:01-[distributed_c10d.py:466]-INFO: Rank 0: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-06 20:12:01-[distributed_c10d.py:466]-INFO: Rank 1: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-06 20:12:01-[distributed_c10d.py:466]-INFO: Rank 3: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-06 20:12:01-[distributed_c10d.py:466]-INFO: Rank 2: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-06 20:12:02-[finetune_with_trainer.py:266]-INFO: ModelArguments(model_path='/data/qiantaotao/base_models/starcoderbase')
2023-09-06 20:12:02-[finetune_with_trainer.py:267]-INFO: TrainingArguments(
_n_gpu=1,
adafactor=False,
adam_beta1=0.9,
adam_beta2=0.999,
adam_epsilon=1e-08,
auto_find_batch_size=False,
bf16=False,
bf16_full_eval=False,
data_seed=42,
dataloader_drop_last=False,
dataloader_num_workers=0,
dataloader_pin_memory=True,
ddp_backend=None,
ddp_broadcast_buffers=None,
ddp_bucket_cap_mb=None,
ddp_find_unused_parameters=None,
ddp_timeout=1800,
debug=[],
deepspeed=/data/chentianyu/silentVuln/LLM/starcoder/ds_config_zero_3.json,
disable_tqdm=False,
do_eval=True,
do_predict=False,
do_train=False,
eval_accumulation_steps=None,
eval_delay=0,
eval_steps=None,
evaluation_strategy=epoch,
fp16=True,
fp16_backend=auto,
fp16_full_eval=False,
fp16_opt_level=O1,
fsdp=[],
fsdp_config={'fsdp_min_num_params': 0, 'xla': False, 'xla_fsdp_grad_ckpt': False},
fsdp_min_num_params=0,
fsdp_transformer_layer_cls_to_wrap=None,
full_determinism=False,
gradient_accumulation_steps=1,
gradient_checkpointing=True,
greater_is_better=False,
group_by_length=False,
half_precision_backend=auto,
hub_model_id=None,
hub_private_repo=False,
hub_strategy=every_save,
hub_token=<HUB_TOKEN>,
ignore_data_skip=False,
include_inputs_for_metrics=True,
jit_mode_eval=False,
label_names=None,
label_smoothing_factor=0.0,
learning_rate=0.0001,
length_column_name=length,
load_best_model_at_end=True,
local_rank=0,
log_level=passive,
log_level_replica=warning,
log_on_each_node=True,
logging_dir=/efs_data/chentianyu/VulFixMiner/checkpoints/exp_3/runs/Sep06_20-12-00_34229c669655,
logging_first_step=False,
logging_nan_inf_filter=True,
logging_steps=10,
logging_strategy=steps,
lr_scheduler_type=linear,
max_grad_norm=1.0,
max_steps=-1,
metric_for_best_model=loss,
mp_parameters=,
no_cuda=False,
num_train_epochs=10,
optim=adamw_torch,
optim_args=None,
output_dir=/efs_data/chentianyu/VulFixMiner/checkpoints/exp_3,
overwrite_output_dir=False,
past_index=-1,
per_device_eval_batch_size=48,
per_device_train_batch_size=16,
prediction_loss_only=False,
push_to_hub=False,
push_to_hub_model_id=None,
push_to_hub_organization=None,
push_to_hub_token=<PUSH_TO_HUB_TOKEN>,
ray_scope=last,
remove_unused_columns=False,
report_to=['tensorboard'],
resume_from_checkpoint=None,
run_name=/efs_data/chentianyu/VulFixMiner/checkpoints/exp_3,
save_on_each_node=False,
save_safetensors=False,
save_steps=500,
save_strategy=epoch,
save_total_limit=None,
seed=42,
sharded_ddp=[],
skip_memory_metrics=True,
tf32=None,
torch_compile=False,
torch_compile_backend=None,
torch_compile_mode=None,
torchdynamo=None,
tpu_metrics_debug=False,
tpu_num_cores=None,
use_ipex=False,
use_legacy_prediction_loop=False,
use_mps_device=False,
warmup_ratio=0.0,
warmup_steps=0,
weight_decay=0.05,
xpu_backend=None,
)
2023-09-06 20:12:02-[finetune_with_trainer.py:268]-INFO: DataArguments(data_dir='/data/chentianyu/VulFixMiner/v1_dataset/v1_context', data_split_path='/data/chentianyu/VulFixMiner/v2_dataset/cross_split.json', datasets_cache_dir='/data/chentianyu/VulFixMiner/cache', max_seq_length=1024, neg_ratio=10, test_only=False, test_checkpoint=None, diff_hunk_col='commit_diff')
2023-09-06 20:12:02-[finetune_with_trainer.py:275]-INFO: GPT2TokenizerFast(name_or_path='/data/qiantaotao/base_models/starcoderbase', vocab_size=49152, model_max_length=1000000000000000019884624838656, is_fast=True, padding_side='right', truncation_side='right', special_tokens={'bos_token': '<|endoftext|>', 'eos_token': '<|endoftext|>', 'unk_token': '<|endoftext|>', 'pad_token': '<|endoftext|>', 'additional_special_tokens': ['<|endoftext|>', '<fim_prefix>', '<fim_middle>', '<fim_suffix>', '<fim_pad>', '<filename>', '<gh_stars>', '<issue_start>', '<issue_comment>', '<issue_closed>', '<jupyter_start>', '<jupyter_text>', '<jupyter_code>', '<jupyter_output>', '<empty_output>', '<commit_before>', '<commit_msg>', '<commit_after>', '<reponame>']}, clean_up_tokenization_spaces=True)
Downloading data files: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 1/1 [00:00<00:00, 10837.99it/s]
Extracting data files: 100%|████████████████████████████████████████████████████████████████████████████████████████████████████████| 1/1 [00:00<00:00, 1556.91it/s]
Setting num_proc from 48 back to 1 for the train split to disable multiprocessing as it only contains one shard.
2023-09-06 20:13:22-[builder.py:1785]-WARNING: Setting num_proc from 48 back to 1 for the train split to disable multiprocessing as it only contains one shard.
Generating train split: 1359 examples [00:00, 28062.38 examples/s]
Downloading data files: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 1/1 [00:00<00:00, 11554.56it/s]
Extracting data files: 100%|████████████████████████████████████████████████████████████████████████████████████████████████████████| 1/1 [00:00<00:00, 1628.86it/s]
Setting num_proc from 48 back to 1 for the train split to disable multiprocessing as it only contains one shard.
2023-09-06 20:14:43-[builder.py:1785]-WARNING: Setting num_proc from 48 back to 1 for the train split to disable multiprocessing as it only contains one shard.
Generating train split: 397415 examples [00:06, 62014.15 examples/s]
Map (num_proc=48): 100%|█████████████████████████████████████████████████████████████████████████████████████████████| 11011/11011 [00:04<00:00, 2205.98 examples/s]
Map (num_proc=48): 100%|████████████████████████████████████████████████████████████████████████████████████████████████| 1232/1232 [00:04<00:00, 252.86 examples/s]
Map (num_proc=48): 100%|█████████████████████████████████████████████████████████████████████████████████████████████| 71381/71381 [00:08<00:00, 8255.35 examples/s]
2023-09-06 20:15:12-[finetune_with_trainer.py:223]-INFO: 
 *** train dataset stats ***
       msg_char_len  num_msg_tokens  diff_char_len  num_diff_tokens         label
count  11011.000000    11011.000000   11011.000000     11011.000000  11011.000000
mean      54.156026       11.959858    3322.488057       928.223231      0.090909
std       37.207057        8.318044    5128.998066      1910.286557      0.287493
min        0.000000        0.000000       0.000000         0.000000      0.000000
25%       32.000000        6.000000     893.000000       252.000000      0.000000
50%       48.000000       10.000000    1870.000000       519.000000      0.000000
75%       68.000000       16.000000    4102.500000      1129.000000      0.000000
max      760.000000      150.000000  227991.000000    141341.000000      1.000000
2023-09-06 20:15:12-[finetune_with_trainer.py:223]-INFO: 
 *** valid dataset stats ***
       msg_char_len  num_msg_tokens  diff_char_len  num_diff_tokens        label
count   1232.000000     1232.000000    1232.000000      1232.000000  1232.000000
mean      52.998377       11.797078    3211.211039       889.133117     0.090909
std       38.828394        8.367050    3973.643364      1135.871537     0.287597
min        0.000000        0.000000       0.000000         0.000000     0.000000
25%       31.000000        6.000000     897.000000       251.000000     0.000000
50%       47.000000       10.000000    1881.500000       524.000000     0.000000
75%       68.000000       15.000000    3985.250000      1089.000000     0.000000
max      628.000000      108.000000   57659.000000     16322.000000     1.000000
2023-09-06 20:15:12-[finetune_with_trainer.py:223]-INFO: 
 *** test dataset stats ***
       msg_char_len  num_msg_tokens  diff_char_len  num_diff_tokens         label
count  71381.000000    71381.000000   71381.000000     71381.000000  71381.000000
mean      54.697356       11.322355    3053.071896       856.732968      0.003446
std       52.838713       37.926470    4287.420648      1311.126467      0.058604
min        0.000000        0.000000       0.000000         0.000000      0.000000
25%       34.000000        6.000000     884.000000       251.000000      0.000000
50%       48.000000       10.000000    1794.000000       503.000000      0.000000
75%       67.000000       15.000000    3871.000000      1076.000000      0.000000
max     9937.000000     9913.000000  354835.000000    101273.000000      1.000000
2023-09-06 20:17:57-[finetune_with_trainer.py:285]-INFO: Loading base model
2023-09-06 20:17:57-[finetune_with_trainer.py:285]-INFO: Loading base model
2023-09-06 20:17:57-[finetune_with_trainer.py:285]-INFO: Loading base model
2023-09-06 20:17:57-[finetune_with_trainer.py:282]-INFO: DatasetDict({
    train: Dataset({
        features: ['input_ids', 'attention_mask', 'label'],
        num_rows: 11011
    })
    valid: Dataset({
        features: ['input_ids', 'attention_mask', 'label'],
        num_rows: 1232
    })
    test: Dataset({
        features: ['input_ids', 'attention_mask', 'label'],
        num_rows: 71381
    })
})
2023-09-06 20:17:57-[finetune_with_trainer.py:285]-INFO: Loading base model
[2023-09-06 20:18:09,067] [INFO] [partition_parameters.py:332:__exit__] finished initializing model - num_params = 485, num_elems = 15.52B
Loading checkpoint shards: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [01:46<00:00, 15.19s/it]
2023-09-06 20:19:55-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Loading checkpoint shards: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [01:46<00:00, 15.19s/it]
Loading checkpoint shards: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [01:46<00:00, 15.19s/it]
2023-09-06 20:19:55-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
2023-09-06 20:19:55-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Loading checkpoint shards: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [01:46<00:00, 15.20s/it]
2023-09-06 20:19:55-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Detected CUDA files, patching ldflags
Emitting ninja build file /root/.cache/torch_extensions/py39_cu117/cpu_adam/build.ninja...
Building extension module cpu_adam...
Allowing ninja to set a default number of workers... (overridable by setting the environment variable MAX_JOBS=N)
ninja: no work to do.
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.0009968280792236 seconds
Loading extension module cpu_adam...
Time to load cpu_adam op: 2.757314443588257 seconds
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Detected CUDA files, patching ldflags
Emitting ninja build file /root/.cache/torch_extensions/py39_cu117/cpu_adam/build.ninja...
Building extension module cpu_adam...
Allowing ninja to set a default number of workers... (overridable by setting the environment variable MAX_JOBS=N)
ninja: no work to do.
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.1570932865142822 seconds
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.477081775665283 seconds
2023-09-06 20:22:15-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 2
2023-09-06 20:22:15-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 3
2023-09-06 20:22:16-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 0
2023-09-06 20:22:16-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 1
2023-09-06 20:22:16-[distributed_c10d.py:466]-INFO: Rank 1: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
2023-09-06 20:22:16-[distributed_c10d.py:466]-INFO: Rank 0: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
2023-09-06 20:22:16-[distributed_c10d.py:466]-INFO: Rank 2: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
2023-09-06 20:22:16-[distributed_c10d.py:466]-INFO: Rank 3: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
Parameter Offload: Total persistent parameters: 2738176 in 324 params
  0%|                                                                                                                                      | 0/1730 [00:00<?, ?it/s]You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
{'loss': 1.8784, 'learning_rate': 0.0001, 'epoch': 0.06}                                                                                                            
{'loss': 1.6907, 'learning_rate': 0.0001, 'epoch': 0.12}                                                                                                            
{'loss': 1.6912, 'learning_rate': 9.971098265895954e-05, 'epoch': 0.17}                                                                                             
  2%|██▏                                                                                                                       | 31/1730 [17:15<16:20:16, 34.62s/it]
{'loss': 1.1501, 'learning_rate': 9.913294797687862e-05, 'epoch': 0.23}                                                                                             
  2%|██▉                                                                                                                       | 42/1730 [23:36<16:13:08, 34.59s/it]{'loss': 1.2445, 'learning_rate': 9.855491329479769e-05, 'epoch': 0.29}                                                                                             
{'loss': 1.3022, 'learning_rate': 9.797687861271677e-05, 'epoch': 0.35}                                                                                             
{'loss': 0.9787, 'learning_rate': 9.739884393063584e-05, 'epoch': 0.4}                                                                                              
  4%|████▉                                                                                                                     | 70/1730 [39:51<16:08:13, 35.00s/it]{'loss': 1.1215, 'learning_rate': 9.682080924855492e-05, 'epoch': 0.46}                                                                                             
{'loss': 1.0195, 'learning_rate': 9.6242774566474e-05, 'epoch': 0.52}                                                                                               
{'loss': 1.0047, 'learning_rate': 9.566473988439308e-05, 'epoch': 0.58}                                                                                             
{'loss': 0.7681, 'learning_rate': 9.508670520231214e-05, 'epoch': 0.64}                                                                                             
{'loss': 0.8185, 'learning_rate': 9.450867052023123e-05, 'epoch': 0.69}                                                                                             
{'loss': 0.705, 'learning_rate': 9.39306358381503e-05, 'epoch': 0.75}                                                                                               
{'loss': 0.4614, 'learning_rate': 9.335260115606937e-05, 'epoch': 0.81}                                                                                             
{'loss': 0.7659, 'learning_rate': 9.277456647398845e-05, 'epoch': 0.87}                                                                                             
{'loss': 0.6873, 'learning_rate': 9.219653179190752e-05, 'epoch': 0.92}                                                                                             
{'loss': 0.6549, 'learning_rate': 9.16184971098266e-05, 'epoch': 0.98}                                                                                              
{'eval_loss': 0.5660417079925537, 'eval_auc': 0.948210299744898, 'eval_f1_best': 0.75, 'eval_f1_threshold': 0.8173828125, 'eval_mcc_best': 0.7302083333333333, 'eval_mcc_threshold': 0.9140625, 'eval_num_samples': 1232, 'eval_runtime': 135.3673, 'eval_samples_per_second': 9.101, 'eval_steps_per_second': 0.052, 'epoch': 1.0}     
 10%|███████████▉                                                                                                           | 173/1730 [1:42:31<15:11:55, 35.14s/it[2023-09-06 22:06:58,906] [WARNING] [stage3.py:1885:step] 1 pytorch allocator cache flushes since last step. this happens when there is high memory pressure and is detrimental to performance. if this is happening frequently consider adjusting settings to reduce memory consumption. If you are unable to make the cache flushes go away consider adding get_accelerator().empty_cache() calls in your training loop to ensure that all ranks flush their caches at the same time
{'loss': 0.5014, 'learning_rate': 9.104046242774567e-05, 'epoch': 1.04}                                                                                             
{'loss': 0.4216, 'learning_rate': 9.046242774566475e-05, 'epoch': 1.1}                                                                                              
{'loss': 0.4163, 'learning_rate': 8.988439306358382e-05, 'epoch': 1.16}                                                                                             
{'loss': 0.5425, 'learning_rate': 8.93063583815029e-05, 'epoch': 1.21}                                                                                              
{'loss': 0.3277, 'learning_rate': 8.872832369942197e-05, 'epoch': 1.27}                                                                                             
{'loss': 0.6293, 'learning_rate': 8.815028901734105e-05, 'epoch': 1.33}                                                                                             
{'loss': 0.4277, 'learning_rate': 8.757225433526012e-05, 'epoch': 1.39}                                                                                             
{'loss': 0.3029, 'learning_rate': 8.69942196531792e-05, 'epoch': 1.45}                                                                                              
{'loss': 0.6036, 'learning_rate': 8.641618497109827e-05, 'epoch': 1.5}                                                                                              
{'loss': 0.33, 'learning_rate': 8.583815028901736e-05, 'epoch': 1.56}                                                                                               
{'loss': 0.2956, 'learning_rate': 8.526011560693643e-05, 'epoch': 1.62}                                                                                             
{'loss': 0.355, 'learning_rate': 8.46820809248555e-05, 'epoch': 1.68}                                                                                               
{'loss': 0.3648, 'learning_rate': 8.410404624277458e-05, 'epoch': 1.73}                                                                                             
{'loss': 0.3488, 'learning_rate': 8.352601156069365e-05, 'epoch': 1.79}                                                                                             
{'loss': 0.34, 'learning_rate': 8.294797687861271e-05, 'epoch': 1.85}                                                                                               
{'loss': 0.6014, 'learning_rate': 8.23699421965318e-05, 'epoch': 1.91}                                                                                              
{'loss': 0.3484, 'learning_rate': 8.179190751445087e-05, 'epoch': 1.97}                                                                                             
{'eval_loss': 0.5562205910682678, 'eval_auc': 0.9587731186224491, 'eval_f1_best': 0.8073394495412844, 'eval_f1_threshold': 0.7724609375, 'eval_mcc_best': 0.7890147788162073, 'eval_mcc_threshold': 0.7724609375, 'eval_num_samples': 1232, 'eval_runtime': 133.6369, 'eval_samples_per_second': 9.219, 'eval_steps_per_second': 0.052, 'epoch': 2.0}
{'loss': 0.2064, 'learning_rate': 8.121387283236995e-05, 'epoch': 2.02}                                                                                             
{'loss': 0.1682, 'learning_rate': 8.063583815028902e-05, 'epoch': 2.08}                                                                                             
{'loss': 0.2762, 'learning_rate': 8.005780346820809e-05, 'epoch': 2.14}                                                                                             
{'loss': 0.1564, 'learning_rate': 7.947976878612717e-05, 'epoch': 2.2}                                                                                              
{'loss': 0.288, 'learning_rate': 7.890173410404624e-05, 'epoch': 2.25}                                                                                              
{'loss': 0.2016, 'learning_rate': 7.832369942196532e-05, 'epoch': 2.31}                                                                                             
{'loss': 0.2534, 'learning_rate': 7.774566473988439e-05, 'epoch': 2.37}                                                                                             
{'loss': 0.1387, 'learning_rate': 7.716763005780347e-05, 'epoch': 2.43}                                                                                             
{'loss': 0.2595, 'learning_rate': 7.658959537572254e-05, 'epoch': 2.49}                                                                                             
{'loss': 0.157, 'learning_rate': 7.601156069364162e-05, 'epoch': 2.54}                                                                                              
{'loss': 0.1052, 'learning_rate': 7.543352601156069e-05, 'epoch': 2.6}                                                                                              
{'loss': 0.2364, 'learning_rate': 7.485549132947977e-05, 'epoch': 2.66}                                                                                             
{'loss': 0.1578, 'learning_rate': 7.427745664739884e-05, 'epoch': 2.72}                                                                                             
{'loss': 0.1109, 'learning_rate': 7.3757225433526e-05, 'epoch': 2.77}                                                                                               
{'loss': 0.4306, 'learning_rate': 7.317919075144509e-05, 'epoch': 2.83}                                                                                             
{'loss': 0.2601, 'learning_rate': 7.260115606936416e-05, 'epoch': 2.89}                                                                                             
{'eval_loss': 1.2251869440078735, 'eval_auc': 0.9613719706632653, 'eval_f1_best': 0.8446601941747574, 'eval_f1_threshold': 0.6474609375, 'eval_mcc_best': 0.834402771383966, 'eval_mcc_threshold': 0.6474609375, 'eval_num_samples': 1232, 'eval_runtime': 133.266, 'eval_samples_per_second': 9.245, 'eval_steps_per_second': 0.053, 'epoch': 3.0}
{'loss': 0.1469, 'learning_rate': 7.144508670520231e-05, 'epoch': 3.01}                                                                                             
{'loss': 0.0189, 'learning_rate': 7.086705202312139e-05, 'epoch': 3.06}                                                                                             
{'loss': 0.0157, 'learning_rate': 7.028901734104046e-05, 'epoch': 3.12}                                                                                             
{'loss': 0.1337, 'learning_rate': 6.971098265895954e-05, 'epoch': 3.18}                                                                                             
{'loss': 0.0112, 'learning_rate': 6.913294797687861e-05, 'epoch': 3.24}                                                                                             
{'loss': 0.0235, 'learning_rate': 6.85549132947977e-05, 'epoch': 3.29}                                                                                              
{'loss': 0.0898, 'learning_rate': 6.797687861271676e-05, 'epoch': 3.35}                                                                                             
{'loss': 0.0215, 'learning_rate': 6.739884393063584e-05, 'epoch': 3.41}                                                                                             
{'loss': 0.2756, 'learning_rate': 6.682080924855491e-05, 'epoch': 3.47}                                                                                             
{'loss': 0.2205, 'learning_rate': 6.624277456647398e-05, 'epoch': 3.53}                                                                                             
{'loss': 0.0678, 'learning_rate': 6.566473988439307e-05, 'epoch': 3.58}                                                                                             
{'loss': 0.0637, 'learning_rate': 6.508670520231213e-05, 'epoch': 3.64}                                                                                             
{'loss': 0.0281, 'learning_rate': 6.450867052023122e-05, 'epoch': 3.7}                                                                                              
{'loss': 0.0554, 'learning_rate': 6.393063583815029e-05, 'epoch': 3.76}                                                                                             
{'loss': 0.0357, 'learning_rate': 6.335260115606937e-05, 'epoch': 3.82}                                                                                             
{'loss': 0.0358, 'learning_rate': 6.277456647398844e-05, 'epoch': 3.87}                                                                                             
{'loss': 0.0457, 'learning_rate': 6.219653179190752e-05, 'epoch': 3.93}                                                                                             
{'loss': 0.0779, 'learning_rate': 6.161849710982659e-05, 'epoch': 3.99}                                                                                             
{'eval_loss': 1.439261794090271, 'eval_auc': 0.9538624043367346, 'eval_f1_best': 0.8557692307692308, 'eval_f1_threshold': 0.98291015625, 'eval_mcc_best': 0.8455434339229622, 'eval_mcc_threshold': 0.98291015625, 'eval_num_samples': 1232, 'eval_runtime': 132.7246, 'eval_samples_per_second': 9.282, 'eval_steps_per_second': 0.053, 'epoch': 4.0}
{'loss': 0.0283, 'learning_rate': 6.104046242774567e-05, 'epoch': 4.05}                                                                                             
{'loss': 0.154, 'learning_rate': 6.046242774566474e-05, 'epoch': 4.1}                                                                                               
{'loss': 0.0179, 'learning_rate': 5.988439306358382e-05, 'epoch': 4.16}                                                                                             
{'loss': 0.1554, 'learning_rate': 5.930635838150289e-05, 'epoch': 4.22}                                                                                             
{'loss': 0.0717, 'learning_rate': 5.8728323699421973e-05, 'epoch': 4.28}                                                                                            
{'loss': 0.004, 'learning_rate': 5.815028901734104e-05, 'epoch': 4.34}                                                                                              
{'loss': 0.0283, 'learning_rate': 5.7572254335260125e-05, 'epoch': 4.39}                                                                                            
{'loss': 0.0117, 'learning_rate': 5.6994219653179194e-05, 'epoch': 4.45}                                                                                            
{'loss': 0.0671, 'learning_rate': 5.6416184971098276e-05, 'epoch': 4.51}                                                                                            
{'loss': 0.1171, 'learning_rate': 5.5838150289017345e-05, 'epoch': 4.57}                                                                                            
{'loss': 0.0064, 'learning_rate': 5.5260115606936414e-05, 'epoch': 4.62}                                                                                            
{'loss': 0.0078, 'learning_rate': 5.46820809248555e-05, 'epoch': 4.68}                                                                                              
{'loss': 0.0331, 'learning_rate': 5.4104046242774566e-05, 'epoch': 4.74}                                                                                            
{'loss': 0.0027, 'learning_rate': 5.352601156069365e-05, 'epoch': 4.8}                                                                                              
{'loss': 0.0054, 'learning_rate': 5.294797687861272e-05, 'epoch': 4.86}                                                                                             
{'loss': 0.0128, 'learning_rate': 5.236994219653179e-05, 'epoch': 4.91}                                                                                             
{'loss': 0.0016, 'learning_rate': 5.179190751445087e-05, 'epoch': 4.97}                                                                                             
{'eval_loss': 1.596268892288208, 'eval_auc': 0.9523198341836734, 'eval_f1_best': 0.8767123287671232, 'eval_f1_threshold': 0.70751953125, 'eval_mcc_best': 0.8670150388346316, 'eval_mcc_threshold': 0.9697265625, 'eval_num_samples': 1232, 'eval_runtime': 132.6139, 'eval_samples_per_second': 9.29, 'eval_steps_per_second': 0.053, 'epoch': 5.0}
{'loss': 0.0027, 'learning_rate': 5.1213872832369944e-05, 'epoch': 5.03}                                                                                            
{'loss': 0.0144, 'learning_rate': 5.063583815028902e-05, 'epoch': 5.09}                                                                                             
{'loss': 0.0164, 'learning_rate': 5.0057803468208096e-05, 'epoch': 5.14}                                                                                            
{'loss': 0.0011, 'learning_rate': 4.9479768786127164e-05, 'epoch': 5.2}                                                                                             
{'loss': 0.0051, 'learning_rate': 4.890173410404624e-05, 'epoch': 5.26}                                                                                             
{'loss': 0.0142, 'learning_rate': 4.8323699421965316e-05, 'epoch': 5.32}                                                                                            
{'loss': 0.0001, 'learning_rate': 4.774566473988439e-05, 'epoch': 5.38}                                                                                             
{'loss': 0.0001, 'learning_rate': 4.716763005780347e-05, 'epoch': 5.43}                                                                                             
{'loss': 0.0, 'learning_rate': 4.658959537572254e-05, 'epoch': 5.49}                                                                                                
{'loss': 0.0011, 'learning_rate': 4.601156069364162e-05, 'epoch': 5.55}                                                                                             
{'loss': 0.0001, 'learning_rate': 4.5433526011560694e-05, 'epoch': 5.61}                                                                                            
{'loss': 0.0019, 'learning_rate': 4.485549132947977e-05, 'epoch': 5.66}                                                                                             
{'loss': 0.0002, 'learning_rate': 4.4277456647398846e-05, 'epoch': 5.72}                                                                                            
{'loss': 0.0001, 'learning_rate': 4.369942196531792e-05, 'epoch': 5.78}                                                                                             
{'loss': 0.0003, 'learning_rate': 4.3121387283237e-05, 'epoch': 5.84}                                                                                               
{'loss': 0.0, 'learning_rate': 4.254335260115607e-05, 'epoch': 5.9}                                                                                                 
{'loss': 0.0, 'learning_rate': 4.196531791907515e-05, 'epoch': 5.95}                                                                                                
{'eval_loss': 2.3082692623138428, 'eval_auc': 0.9486447704081633, 'eval_f1_best': 0.8847926267281105, 'eval_f1_threshold': 0.4580078125, 'eval_mcc_best': 0.8742263841935505, 'eval_mcc_threshold': 0.4580078125, 'eval_num_samples': 1232, 'eval_runtime': 132.5454, 'eval_samples_per_second': 9.295, 'eval_steps_per_second': 0.053, 'epoch': 6.0}
{'loss': 0.0006, 'learning_rate': 4.1387283236994224e-05, 'epoch': 6.01}                                                                                            
{'loss': 0.0002, 'learning_rate': 4.08092485549133e-05, 'epoch': 6.07}                                                                                              
{'loss': 0.0001, 'learning_rate': 4.0231213872832376e-05, 'epoch': 6.13}                                                                                            
{'loss': 0.0054, 'learning_rate': 3.965317919075145e-05, 'epoch': 6.18}                                                                                             
{'loss': 0.0001, 'learning_rate': 3.907514450867053e-05, 'epoch': 6.24}                                                                                             
{'loss': 0.0, 'learning_rate': 3.8497109826589596e-05, 'epoch': 6.3}                                                                                                
{'loss': 0.0, 'learning_rate': 3.791907514450867e-05, 'epoch': 6.36}                                                                                                
{'loss': 0.0001, 'learning_rate': 3.734104046242775e-05, 'epoch': 6.42}                                                                                             
{'loss': 0.0, 'learning_rate': 3.676300578034682e-05, 'epoch': 6.47}                                                                                                
{'loss': 0.0147, 'learning_rate': 3.61849710982659e-05, 'epoch': 6.53}                                                                                              
{'loss': 0.0011, 'learning_rate': 3.5606936416184975e-05, 'epoch': 6.59}                                                                                            
{'loss': 0.0001, 'learning_rate': 3.502890173410405e-05, 'epoch': 6.65}                                                                                             
{'loss': 0.0001, 'learning_rate': 3.445086705202312e-05, 'epoch': 6.71}                                                                                             
{'loss': 0.0003, 'learning_rate': 3.3872832369942195e-05, 'epoch': 6.76}                                                                                            
{'loss': 0.0155, 'learning_rate': 3.329479768786127e-05, 'epoch': 6.82}                                                                                             
{'loss': 0.0029, 'learning_rate': 3.2716763005780346e-05, 'epoch': 6.88}                                                                                            
{'loss': 0.0, 'learning_rate': 3.213872832369942e-05, 'epoch': 6.94}                                                                                                
{'loss': 0.12, 'learning_rate': 3.15606936416185e-05, 'epoch': 6.99}                                                                                                
{'eval_loss': 2.0234735012054443, 'eval_auc': 0.9511639030612246, 'eval_f1_best': 0.875, 'eval_f1_threshold': 0.9912109375, 'eval_mcc_best': 0.8666102012460711, 'eval_mcc_threshold': 0.9912109375, 'eval_num_samples': 1232, 'eval_runtime': 132.5806, 'eval_samples_per_second': 9.292, 'eval_steps_per_second': 0.053, 'epoch': 7.0}
{'loss': 0.0, 'learning_rate': 3.0982658959537573e-05, 'epoch': 7.05}                                                                                               
{'loss': 0.0, 'learning_rate': 3.040462427745665e-05, 'epoch': 7.11}                                                                                                
{'loss': 0.0, 'learning_rate': 2.9826589595375725e-05, 'epoch': 7.17}                                                                                               
{'loss': 0.0001, 'learning_rate': 2.92485549132948e-05, 'epoch': 7.23}                                                                                              
{'loss': 0.0001, 'learning_rate': 2.8670520231213876e-05, 'epoch': 7.28}                                                                                            
{'loss': 0.0001, 'learning_rate': 2.8092485549132952e-05, 'epoch': 7.34}                                                                                            
{'loss': 0.0, 'learning_rate': 2.751445086705202e-05, 'epoch': 7.4}                                                                                                 
{'loss': 0.0001, 'learning_rate': 2.6936416184971097e-05, 'epoch': 7.46}                                                                                            
{'loss': 0.0007, 'learning_rate': 2.6358381502890172e-05, 'epoch': 7.51}                                                                                            
{'loss': 0.0105, 'learning_rate': 2.5780346820809248e-05, 'epoch': 7.57}                                                                                            
{'loss': 0.0, 'learning_rate': 2.5202312138728324e-05, 'epoch': 7.63}                                                                                               
{'loss': 0.0, 'learning_rate': 2.46242774566474e-05, 'epoch': 7.69}                                                                                                 
{'loss': 0.0026, 'learning_rate': 2.4046242774566475e-05, 'epoch': 7.75}                                                                                            
{'loss': 0.0002, 'learning_rate': 2.346820809248555e-05, 'epoch': 7.8}                                                                                              
 78%|████████████████████████████████████████████████████████████████████████████████████████████▎                         | 1354/1730 [13:40:28<3:39:57, 35.10s/it]{'loss': 0.0024, 'learning_rate': 2.2890173410404627e-05, 'epoch': 7.86}                                                                                            
{'loss': 0.0084, 'learning_rate': 2.23121387283237e-05, 'epoch': 7.92}                                                                                              
{'loss': 0.0, 'learning_rate': 2.1734104046242775e-05, 'epoch': 7.98}                                                                                               
{'eval_loss': 2.439391613006592, 'eval_auc': 0.9447544642857143, 'eval_f1_best': 0.8792270531400966, 'eval_f1_threshold': 0.68359375, 'eval_mcc_best': 0.8717383711912933, 'eval_mcc_threshold': 0.68359375, 'eval_num_samples': 1232, 'eval_runtime': 132.6358, 'eval_samples_per_second': 9.289, 'eval_steps_per_second': 0.053, 'epoch': 8.0}
{'loss': 0.0001, 'learning_rate': 2.115606936416185e-05, 'epoch': 8.03}                                                                                             
{'loss': 0.0, 'learning_rate': 2.0578034682080926e-05, 'epoch': 8.09}                                                                                               
{'loss': 0.0, 'learning_rate': 2e-05, 'epoch': 8.15}                                                                                                                
 82%|████████████████████████████████████████████████████████████████████████████████████████████████▋                     | 1417/1730 [14:21:04<3:01:52, 34.87s/it]{'loss': 0.0, 'learning_rate': 1.9421965317919074e-05, 'epoch': 8.21}                                                                                               
{'loss': 0.0, 'learning_rate': 1.884393063583815e-05, 'epoch': 8.27}                                                                                                
{'loss': 0.0014, 'learning_rate': 1.8265895953757225e-05, 'epoch': 8.32}                                                                                            
{'loss': 0.0, 'learning_rate': 1.76878612716763e-05, 'epoch': 8.38}                                                                                                 
{'loss': 0.0081, 'learning_rate': 1.7109826589595377e-05, 'epoch': 8.44}                                                                                            
{'loss': 0.0001, 'learning_rate': 1.6531791907514452e-05, 'epoch': 8.5}                                                                                             
 85%|████████████████████████████████████████████████████████████████████████████████████████████████████▎                 | 1471/1730 [14:52:42<2:31:10, 35.02s/it]{'loss': 0.0, 'learning_rate': 1.5953757225433528e-05, 'epoch': 8.55}                                                                                               
{'loss': 0.0047, 'learning_rate': 1.5375722543352604e-05, 'epoch': 8.61}                                                                                            
{'loss': 0.0001, 'learning_rate': 1.4797687861271678e-05, 'epoch': 8.67}                                                                                            
{'loss': 0.0, 'learning_rate': 1.4219653179190754e-05, 'epoch': 8.73}                                                                                               
{'loss': 0.0117, 'learning_rate': 1.3641618497109826e-05, 'epoch': 8.79}                                                                                            
{'loss': 0.0, 'learning_rate': 1.3063583815028902e-05, 'epoch': 8.84}                                                                                               
{'loss': 0.0, 'learning_rate': 1.2485549132947977e-05, 'epoch': 8.9}                                                                                                
{'loss': 0.0, 'learning_rate': 1.1907514450867053e-05, 'epoch': 8.96}                                                                                               
{'eval_loss': 2.3035342693328857, 'eval_auc': 0.9444754464285715, 'eval_f1_best': 0.8792270531400966, 'eval_f1_threshold': 0.9091796875, 'eval_mcc_best': 0.8717383711912933, 'eval_mcc_threshold': 0.9091796875, 'eval_num_samples': 1232, 'eval_runtime': 132.3714, 'eval_samples_per_second': 9.307, 'eval_steps_per_second': 0.053, 'epoch': 9.0}
{'loss': 0.0008, 'learning_rate': 1.1329479768786127e-05, 'epoch': 9.02}                                                                                            
{'loss': 0.0019, 'learning_rate': 1.0751445086705203e-05, 'epoch': 9.08}                                                                                            
{'loss': 0.0, 'learning_rate': 1.0173410404624278e-05, 'epoch': 9.13}                                                                                               
{'loss': 0.0, 'learning_rate': 9.595375722543352e-06, 'epoch': 9.19}                                                                                                
{'loss': 0.0006, 'learning_rate': 9.017341040462428e-06, 'epoch': 9.25}                                                                                             
{'loss': 0.0075, 'learning_rate': 8.439306358381504e-06, 'epoch': 9.31}                                                                                             
{'loss': 0.0, 'learning_rate': 7.861271676300578e-06, 'epoch': 9.36}                                                                                                
{'loss': 0.0001, 'learning_rate': 7.2832369942196544e-06, 'epoch': 9.42}                                                                                            
{'loss': 0.0001, 'learning_rate': 6.7052023121387284e-06, 'epoch': 9.48}                                                                                            
{'loss': 0.0001, 'learning_rate': 6.127167630057803e-06, 'epoch': 9.54}                                                                                             
{'loss': 0.0, 'learning_rate': 5.549132947976879e-06, 'epoch': 9.6}                                                                                                 
{'loss': 0.0, 'learning_rate': 4.971098265895955e-06, 'epoch': 9.65}                                                                                                
{'loss': 0.0, 'learning_rate': 4.393063583815029e-06, 'epoch': 9.71}                                                                                                
{'loss': 0.0, 'learning_rate': 3.815028901734104e-06, 'epoch': 9.77}                                                                                                
{'loss': 0.0062, 'learning_rate': 3.2369942196531793e-06, 'epoch': 9.83}                                                                                            
{'loss': 0.0, 'learning_rate': 2.6589595375722546e-06, 'epoch': 9.88}                                                                                               
{'loss': 0.0116, 'learning_rate': 2.0809248554913294e-06, 'epoch': 9.94}                                                                                            
{'loss': 0.0001, 'learning_rate': 1.5028901734104047e-06, 'epoch': 10.0}                                                                                            
{'eval_loss': 2.1966965198516846, 'eval_auc': 0.9481823979591836, 'eval_f1_best': 0.8858447488584474, 'eval_f1_threshold': 0.27392578125, 'eval_mcc_best': 0.874989986591569, 'eval_mcc_threshold': 0.27392578125, 'eval_num_samples': 1232, 'eval_runtime': 132.6903, 'eval_samples_per_second': 9.285, 'eval_steps_per_second': 0.053, 'epoch': 10.0}
{'train_runtime': 63529.7184, 'train_samples_per_second': 1.733, 'train_steps_per_second': 0.027, 'train_loss': 0.18016901585580297, 'epoch': 10.0}                 
100%|████████████████████████████████████████████████████████████████████████████████████████████████████████████████████████| 1730/1730 [17:38:49<00:00, 36.72s/it]
  2%|██▎                                                                                                                          | 7/372 [01:54<1:49:30, 18.00s/it] 60%|██████████████████████████████████████████████████████████████████████████                                                 | 224/372 [1:11:10<47:19, 19.19s/it] 95%|█████████████████████████████████████████████████████████████████████████████████████████████████████████████████████      | 354/372 [1:52:41<05:46, 19.22s/it]100%|███████████████████████████████████████████████████████████████████████████████████████████████████████████████████████████| 372/372 [1:58:26<00:00, 19.19s/it]100%|███████████████████████████████████████████████████████████████████████████████████████████████████████████████████████████| 372/372 [1:59:33<00:00, 19.28s/it]
{'test_loss': 0.25562360882759094, 'test_auc': 0.9308628503801029, 'test_f1_best': 0.3166023166023166, 'test_f1_threshold': 0.98291015625, 'test_mcc_best': 0.3145192556216451, 'test_mcc_threshold': 0.98291015625, 'test_num_samples': 71381, 'test_runtime': 7192.1357, 'test_samples_per_second': 9.925, 'test_steps_per_second': 0.052}
[2023-09-07 16:01:02,937] [INFO] [launch.py:347:main] Process 5494 exits successfully.
[2023-09-07 16:01:04,940] [INFO] [launch.py:347:main] Process 5493 exits successfully.
[2023-09-07 16:01:06,942] [INFO] [launch.py:347:main] Process 5492 exits successfully.
[2023-09-07 16:01:10,946] [INFO] [launch.py:347:main] Process 5491 exits successfully.
















(PyTorch-2.0.0) root@34229c669655:/data/chentianyu/silentVuln/LLM/starcoder/scripts# ./run_exp_5.sh 
[2023-09-07 17:40:19,016] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-07 17:40:21,101] [WARNING] [runner.py:201:fetch_hostfile] Unable to find hostfile, will proceed with training with local resources only.
[2023-09-07 17:40:21,184] [INFO] [runner.py:567:main] cmd = /home/ma-user/anaconda3/envs/PyTorch-2.0.0/bin/python -u -m deepspeed.launcher.launch --world_info=eyJsb2NhbGhvc3QiOiBbNCwgNSwgNiwgN119 --master_addr=127.0.0.1 --master_port=27987 --enable_each_rank_log=None /data/chentianyu/silentVuln/LLM/starcoder/finetune_with_trainer.py --model_path /data/qiantaotao/base_models/starcoderbase --deepspeed /data/chentianyu/silentVuln/LLM/starcoder/ds_config_zero_3.json --output_dir /efs_data/chentianyu/VulFixMiner/checkpoints/exp_5 --per_device_eval_batch_size 12 --per_device_train_batch_size 4 --num_train_epochs 10 --logging_steps 10 --gradient_checkpointing true --remove_unused_columns false --fp16 true --load_best_model_at_end true --include_inputs_for_metrics true --data_seed 42 --learning_rate 1e-4 --weight_decay 0.05 --save_strategy epoch --evaluation_strategy epoch --optim adamw_torch --data_dir /data/chentianyu/VulFixMiner/v1_dataset/v1_context --data_split_path /data/chentianyu/VulFixMiner/v2_dataset/cross_split.json --datasets_cache_dir /data/chentianyu/VulFixMiner/cache --max_seq_length 2048 --neg_ratio 10 --test_only false --diff_hunk_col commit_diff --r 16 --lora_alpha 32 --lora_dropout 0.05
[2023-09-07 17:40:23,281] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-07 17:40:25,564] [INFO] [launch.py:138:main] 0 NCCL_VERSION=2.13.4-1
[2023-09-07 17:40:25,564] [INFO] [launch.py:145:main] WORLD INFO DICT: {'localhost': [4, 5, 6, 7]}
[2023-09-07 17:40:25,564] [INFO] [launch.py:151:main] nnodes=1, num_local_procs=4, node_rank=0
[2023-09-07 17:40:25,564] [INFO] [launch.py:162:main] global_rank_mapping=defaultdict(<class 'list'>, {'localhost': [0, 1, 2, 3]})
[2023-09-07 17:40:25,564] [INFO] [launch.py:163:main] dist_world_size=4
[2023-09-07 17:40:25,564] [INFO] [launch.py:165:main] Setting CUDA_VISIBLE_DEVICES=4,5,6,7
[2023-09-07 17:40:29,801] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-07 17:40:29,834] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-07 17:40:29,859] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-07 17:40:29,881] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-07 17:40:33,579] [INFO] [comm.py:631:init_distributed] cdb=None
[2023-09-07 17:40:33,592] [INFO] [comm.py:631:init_distributed] cdb=None
[2023-09-07 17:40:33,649] [INFO] [comm.py:631:init_distributed] cdb=None
[2023-09-07 17:40:33,797] [INFO] [comm.py:631:init_distributed] cdb=None
[2023-09-07 17:40:33,797] [INFO] [comm.py:662:init_distributed] Initializing TorchBackend in DeepSpeed with backend nccl
2023-09-07 17:40:34-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 2
2023-09-07 17:40:34-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 1
2023-09-07 17:40:34-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 3
2023-09-07 17:40:34-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 0
2023-09-07 17:40:34-[distributed_c10d.py:466]-INFO: Rank 0: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-07 17:40:34-[distributed_c10d.py:466]-INFO: Rank 2: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-07 17:40:34-[distributed_c10d.py:466]-INFO: Rank 1: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-07 17:40:34-[distributed_c10d.py:466]-INFO: Rank 3: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-07 17:40:35-[finetune_with_trainer.py:266]-INFO: ModelArguments(model_path='/data/qiantaotao/base_models/starcoderbase')
2023-09-07 17:40:35-[finetune_with_trainer.py:267]-INFO: TrainingArguments(
_n_gpu=1,
adafactor=False,
adam_beta1=0.9,
adam_beta2=0.999,
adam_epsilon=1e-08,
auto_find_batch_size=False,
bf16=False,
bf16_full_eval=False,
data_seed=42,
dataloader_drop_last=False,
dataloader_num_workers=0,
dataloader_pin_memory=True,
ddp_backend=None,
ddp_broadcast_buffers=None,
ddp_bucket_cap_mb=None,
ddp_find_unused_parameters=None,
ddp_timeout=1800,
debug=[],
deepspeed=/data/chentianyu/silentVuln/LLM/starcoder/ds_config_zero_3.json,
disable_tqdm=False,
do_eval=True,
do_predict=False,
do_train=False,
eval_accumulation_steps=None,
eval_delay=0,
eval_steps=None,
evaluation_strategy=epoch,
fp16=True,
fp16_backend=auto,
fp16_full_eval=False,
fp16_opt_level=O1,
fsdp=[],
fsdp_config={'fsdp_min_num_params': 0, 'xla': False, 'xla_fsdp_grad_ckpt': False},
fsdp_min_num_params=0,
fsdp_transformer_layer_cls_to_wrap=None,
full_determinism=False,
gradient_accumulation_steps=1,
gradient_checkpointing=True,
greater_is_better=False,
group_by_length=False,
half_precision_backend=auto,
hub_model_id=None,
hub_private_repo=False,
hub_strategy=every_save,
hub_token=<HUB_TOKEN>,
ignore_data_skip=False,
include_inputs_for_metrics=True,
jit_mode_eval=False,
label_names=None,
label_smoothing_factor=0.0,
learning_rate=0.0001,
length_column_name=length,
load_best_model_at_end=True,
local_rank=0,
log_level=passive,
log_level_replica=warning,
log_on_each_node=True,
logging_dir=/efs_data/chentianyu/VulFixMiner/checkpoints/exp_5/runs/Sep07_17-40-33_34229c669655,
logging_first_step=False,
logging_nan_inf_filter=True,
logging_steps=10,
logging_strategy=steps,
lr_scheduler_type=linear,
max_grad_norm=1.0,
max_steps=-1,
metric_for_best_model=loss,
mp_parameters=,
no_cuda=False,
num_train_epochs=10,
optim=adamw_torch,
optim_args=None,
output_dir=/efs_data/chentianyu/VulFixMiner/checkpoints/exp_5,
overwrite_output_dir=False,
past_index=-1,
per_device_eval_batch_size=12,
per_device_train_batch_size=4,
prediction_loss_only=False,
push_to_hub=False,
push_to_hub_model_id=None,
push_to_hub_organization=None,
push_to_hub_token=<PUSH_TO_HUB_TOKEN>,
ray_scope=last,
remove_unused_columns=False,
report_to=['tensorboard'],
resume_from_checkpoint=None,
run_name=/efs_data/chentianyu/VulFixMiner/checkpoints/exp_5,
save_on_each_node=False,
save_safetensors=False,
save_steps=500,
save_strategy=epoch,
save_total_limit=None,
seed=42,
sharded_ddp=[],
skip_memory_metrics=True,
tf32=None,
torch_compile=False,
torch_compile_backend=None,
torch_compile_mode=None,
torchdynamo=None,
tpu_metrics_debug=False,
tpu_num_cores=None,
use_ipex=False,
use_legacy_prediction_loop=False,
use_mps_device=False,
warmup_ratio=0.0,
warmup_steps=0,
weight_decay=0.05,
xpu_backend=None,
)
2023-09-07 17:40:35-[finetune_with_trainer.py:268]-INFO: DataArguments(data_dir='/data/chentianyu/VulFixMiner/v1_dataset/v1_context', data_split_path='/data/chentianyu/VulFixMiner/v2_dataset/cross_split.json', datasets_cache_dir='/data/chentianyu/VulFixMiner/cache', max_seq_length=2048, neg_ratio=10, test_only=False, test_checkpoint=None, diff_hunk_col='commit_diff')
2023-09-07 17:40:35-[finetune_with_trainer.py:275]-INFO: GPT2TokenizerFast(name_or_path='/data/qiantaotao/base_models/starcoderbase', vocab_size=49152, model_max_length=1000000000000000019884624838656, is_fast=True, padding_side='right', truncation_side='right', special_tokens={'bos_token': '<|endoftext|>', 'eos_token': '<|endoftext|>', 'unk_token': '<|endoftext|>', 'pad_token': '<|endoftext|>', 'additional_special_tokens': ['<|endoftext|>', '<fim_prefix>', '<fim_middle>', '<fim_suffix>', '<fim_pad>', '<filename>', '<gh_stars>', '<issue_start>', '<issue_comment>', '<issue_closed>', '<jupyter_start>', '<jupyter_text>', '<jupyter_code>', '<jupyter_output>', '<empty_output>', '<commit_before>', '<commit_msg>', '<commit_after>', '<reponame>']}, clean_up_tokenization_spaces=True)
2023-09-07 17:43:18-[finetune_with_trainer.py:223]-INFO: 
 *** train dataset stats ***
       msg_char_len  num_msg_tokens  diff_char_len  num_diff_tokens         label
count  11011.000000    11011.000000   11011.000000     11011.000000  11011.000000
mean      54.156026       11.959858    3322.488057       928.223231      0.090909
std       37.207057        8.318044    5128.998066      1910.286557      0.287493
min        0.000000        0.000000       0.000000         0.000000      0.000000
25%       32.000000        6.000000     893.000000       252.000000      0.000000
50%       48.000000       10.000000    1870.000000       519.000000      0.000000
75%       68.000000       16.000000    4102.500000      1129.000000      0.000000
max      760.000000      150.000000  227991.000000    141341.000000      1.000000
2023-09-07 17:43:18-[finetune_with_trainer.py:223]-INFO: 
 *** valid dataset stats ***
       msg_char_len  num_msg_tokens  diff_char_len  num_diff_tokens        label
count   1232.000000     1232.000000    1232.000000      1232.000000  1232.000000
mean      52.998377       11.797078    3211.211039       889.133117     0.090909
std       38.828394        8.367050    3973.643364      1135.871537     0.287597
min        0.000000        0.000000       0.000000         0.000000     0.000000
25%       31.000000        6.000000     897.000000       251.000000     0.000000
50%       47.000000       10.000000    1881.500000       524.000000     0.000000
75%       68.000000       15.000000    3985.250000      1089.000000     0.000000
max      628.000000      108.000000   57659.000000     16322.000000     1.000000
2023-09-07 17:43:18-[finetune_with_trainer.py:223]-INFO: 
 *** test dataset stats ***
       msg_char_len  num_msg_tokens  diff_char_len  num_diff_tokens         label
count  71381.000000    71381.000000   71381.000000     71381.000000  71381.000000
mean      54.697356       11.322355    3053.071896       856.732968      0.003446
std       52.838713       37.926470    4287.420648      1311.126467      0.058604
min        0.000000        0.000000       0.000000         0.000000      0.000000
25%       34.000000        6.000000     884.000000       251.000000      0.000000
50%       48.000000       10.000000    1794.000000       503.000000      0.000000
75%       67.000000       15.000000    3871.000000      1076.000000      0.000000
max     9937.000000     9913.000000  354835.000000    101273.000000      1.000000
2023-09-07 17:46:06-[finetune_with_trainer.py:285]-INFO: Loading base model
2023-09-07 17:46:06-[finetune_with_trainer.py:285]-INFO: Loading base model
2023-09-07 17:46:06-[finetune_with_trainer.py:285]-INFO: Loading base model
2023-09-07 17:46:06-[finetune_with_trainer.py:282]-INFO: DatasetDict({
    train: Dataset({
        features: ['input_ids', 'attention_mask', 'label'],
        num_rows: 11011
    })
    valid: Dataset({
        features: ['input_ids', 'attention_mask', 'label'],
        num_rows: 1232
    })
    test: Dataset({
        features: ['input_ids', 'attention_mask', 'label'],
        num_rows: 71381
    })
})
2023-09-07 17:46:06-[finetune_with_trainer.py:285]-INFO: Loading base model
[2023-09-07 17:46:26,392] [INFO] [partition_parameters.py:332:__exit__] finished initializing model - num_params = 485, num_elems = 15.52B
Loading checkpoint shards: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [01:20<00:00, 11.57s/it]
Loading checkpoint shards: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [01:21<00:00, 11.57s/it]
2023-09-07 17:47:47-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
2023-09-07 17:47:47-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Loading checkpoint shards: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [01:21<00:00, 11.57s/it]
2023-09-07 17:47:47-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Loading checkpoint shards: 100%|██████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [01:21<00:00, 11.58s/it]
2023-09-07 17:47:47-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Detected CUDA files, patching ldflags
Emitting ninja build file /root/.cache/torch_extensions/py39_cu117/cpu_adam/build.ninja...
Building extension module cpu_adam...
Allowing ninja to set a default number of workers... (overridable by setting the environment variable MAX_JOBS=N)
ninja: no work to do.
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.238807439804077 seconds
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.3497302532196045 seconds
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Detected CUDA files, patching ldflags
Emitting ninja build file /root/.cache/torch_extensions/py39_cu117/cpu_adam/build.ninja...
Building extension module cpu_adam...
Allowing ninja to set a default number of workers... (overridable by setting the environment variable MAX_JOBS=N)
ninja: no work to do.
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.338559865951538 seconds
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.3118488788604736 seconds
2023-09-07 17:50:27-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 0
2023-09-07 17:50:27-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 1
2023-09-07 17:50:29-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 3
2023-09-07 17:50:29-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 2
2023-09-07 17:50:29-[distributed_c10d.py:466]-INFO: Rank 2: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
2023-09-07 17:50:29-[distributed_c10d.py:466]-INFO: Rank 3: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
2023-09-07 17:50:29-[distributed_c10d.py:466]-INFO: Rank 0: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
2023-09-07 17:50:29-[distributed_c10d.py:466]-INFO: Rank 1: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
Parameter Offload: Total persistent parameters: 2738176 in 324 params
  0%|                                                                                                                                      | 0/6890 [00:00<?, ?it/s]You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
  0%|▏                                                                                                                          | 8/6890 [04:47<66:16:21, 34.67s/it]{'loss': 1.7643, 'learning_rate': 0.0001, 'epoch': 0.01}                                                                                                            
  0%|▏                                                                                                                         | 13/6890 [07:38<65:10:15, 34.12s/it]{'loss': 2.2202, 'learning_rate': 0.0001, 'epoch': 0.03}                                                                                                            
{'loss': 1.7127, 'learning_rate': 9.992743105950654e-05, 'epoch': 0.04}                                                                                             
{'loss': 1.0642, 'learning_rate': 9.97822931785196e-05, 'epoch': 0.06}                                                                                              
{'loss': 1.4389, 'learning_rate': 9.965166908563135e-05, 'epoch': 0.07}                                                                                             
{'loss': 1.1279, 'learning_rate': 9.950653120464442e-05, 'epoch': 0.09}                                                                                             
{'loss': 1.2858, 'learning_rate': 9.936139332365748e-05, 'epoch': 0.1}                                                                                              
{'loss': 1.3915, 'learning_rate': 9.921625544267055e-05, 'epoch': 0.12}                                                                                             
{'loss': 1.2233, 'learning_rate': 9.90711175616836e-05, 'epoch': 0.13}                                                                                              
{'loss': 1.2448, 'learning_rate': 9.892597968069667e-05, 'epoch': 0.15}                                                                                             
{'loss': 1.2846, 'learning_rate': 9.878084179970973e-05, 'epoch': 0.16}                                                                                             
{'loss': 1.1952, 'learning_rate': 9.863570391872278e-05, 'epoch': 0.17}                                                                                             
{'loss': 0.9017, 'learning_rate': 9.849056603773585e-05, 'epoch': 0.19}                                                                                             
{'loss': 1.0026, 'learning_rate': 9.834542815674891e-05, 'epoch': 0.2}                                                                                              
{'loss': 1.1324, 'learning_rate': 9.820029027576198e-05, 'epoch': 0.22}                                                                                             
{'loss': 0.989, 'learning_rate': 9.805515239477504e-05, 'epoch': 0.23}                                                                                              
{'loss': 0.8708, 'learning_rate': 9.791001451378811e-05, 'epoch': 0.25}                                                                                             
{'loss': 0.9658, 'learning_rate': 9.776487663280116e-05, 'epoch': 0.26}                                                                                             
{'loss': 1.0031, 'learning_rate': 9.761973875181423e-05, 'epoch': 0.28}                                                                                             
{'loss': 0.8972, 'learning_rate': 9.747460087082729e-05, 'epoch': 0.29}                                                                                             
{'loss': 1.4141, 'learning_rate': 9.732946298984034e-05, 'epoch': 0.3}                                                                                              
{'loss': 0.666, 'learning_rate': 9.718432510885341e-05, 'epoch': 0.32}                                                                                              
{'loss': 0.8159, 'learning_rate': 9.703918722786647e-05, 'epoch': 0.33}                                                                                             
{'loss': 0.486, 'learning_rate': 9.689404934687954e-05, 'epoch': 0.35}                                                                                              
{'loss': 1.2066, 'learning_rate': 9.67489114658926e-05, 'epoch': 0.36}                                                                                              
{'loss': 0.8672, 'learning_rate': 9.660377358490567e-05, 'epoch': 0.38}                                                                                             
{'loss': 0.9088, 'learning_rate': 9.645863570391874e-05, 'epoch': 0.39}                                                                                             
{'loss': 1.7004, 'learning_rate': 9.631349782293179e-05, 'epoch': 0.41}                                                                                             
{'loss': 0.6629, 'learning_rate': 9.616835994194485e-05, 'epoch': 0.42}                                                                                             
{'loss': 0.3806, 'learning_rate': 9.602322206095792e-05, 'epoch': 0.44}                                                                                             
{'loss': 3.4193, 'learning_rate': 9.587808417997097e-05, 'epoch': 0.45}                                                                                             
{'loss': 0.8169, 'learning_rate': 9.573294629898403e-05, 'epoch': 0.46}                                                                                             
{'loss': 0.5656, 'learning_rate': 9.55878084179971e-05, 'epoch': 0.48}                                                                                              
{'loss': 1.2396, 'learning_rate': 9.544267053701017e-05, 'epoch': 0.49}                                                                                             
{'loss': 1.9251, 'learning_rate': 9.529753265602323e-05, 'epoch': 0.51}                                                                                             
{'loss': 2.0757, 'learning_rate': 9.51523947750363e-05, 'epoch': 0.52}                                                                                              
{'loss': 1.2668, 'learning_rate': 9.500725689404936e-05, 'epoch': 0.54}                                                                                             
{'loss': 0.4782, 'learning_rate': 9.486211901306241e-05, 'epoch': 0.55}                                                                                             
{'loss': 1.541, 'learning_rate': 9.471698113207548e-05, 'epoch': 0.57}                                                                                              
{'loss': 0.9881, 'learning_rate': 9.457184325108854e-05, 'epoch': 0.58}                                                                                             
{'loss': 0.741, 'learning_rate': 9.44267053701016e-05, 'epoch': 0.6}                                                                                                
{'loss': 0.2414, 'learning_rate': 9.428156748911466e-05, 'epoch': 0.61}                                                                                             
{'loss': 0.9186, 'learning_rate': 9.413642960812773e-05, 'epoch': 0.62}                                                                                             
{'loss': 0.4365, 'learning_rate': 9.399129172714078e-05, 'epoch': 0.64}                                                                                             
{'loss': 2.4559, 'learning_rate': 9.384615384615386e-05, 'epoch': 0.65}                                                                                             
{'loss': 0.4391, 'learning_rate': 9.370101596516692e-05, 'epoch': 0.67}                                                                                             
{'loss': 1.2358, 'learning_rate': 9.355587808417997e-05, 'epoch': 0.68}                                                                                             
{'loss': 0.9771, 'learning_rate': 9.341074020319304e-05, 'epoch': 0.7}                                                                                              
{'loss': 1.1745, 'learning_rate': 9.32656023222061e-05, 'epoch': 0.71}                                                                                              
{'loss': 0.8801, 'learning_rate': 9.312046444121916e-05, 'epoch': 0.73}                                                                                             
{'loss': 0.5517, 'learning_rate': 9.297532656023222e-05, 'epoch': 0.74}                                                                                             
{'loss': 2.0675, 'learning_rate': 9.283018867924529e-05, 'epoch': 0.75}                                                                                             
{'loss': 0.7776, 'learning_rate': 9.268505079825835e-05, 'epoch': 0.77}                                                                                             
{'loss': 0.8358, 'learning_rate': 9.25399129172714e-05, 'epoch': 0.78}                                                                                              
{'loss': 0.8163, 'learning_rate': 9.239477503628447e-05, 'epoch': 0.8}                                                                                              
{'loss': 0.6094, 'learning_rate': 9.224963715529755e-05, 'epoch': 0.81}                                                                                             
{'loss': 0.9825, 'learning_rate': 9.21044992743106e-05, 'epoch': 0.83}                                                                                              
{'loss': 0.7178, 'learning_rate': 9.195936139332366e-05, 'epoch': 0.84}                                                                                             
{'loss': 1.2533, 'learning_rate': 9.181422351233673e-05, 'epoch': 0.86}                                                                                             
{'loss': 0.6138, 'learning_rate': 9.166908563134978e-05, 'epoch': 0.87}                                                                                             
{'loss': 1.4206, 'learning_rate': 9.152394775036285e-05, 'epoch': 0.89}                                                                                             
{'loss': 0.796, 'learning_rate': 9.137880986937591e-05, 'epoch': 0.9}                                                                                               
{'loss': 1.0292, 'learning_rate': 9.123367198838896e-05, 'epoch': 0.91}                                                                                             
{'loss': 1.1653, 'learning_rate': 9.108853410740203e-05, 'epoch': 0.93}                                                                                             
{'loss': 1.2461, 'learning_rate': 9.09433962264151e-05, 'epoch': 0.94}                                                                                              
{'loss': 1.7863, 'learning_rate': 9.079825834542816e-05, 'epoch': 0.96}                                                                                             
{'loss': 1.033, 'learning_rate': 9.065312046444123e-05, 'epoch': 0.97}                                                                                              
{'loss': 0.9915, 'learning_rate': 9.050798258345429e-05, 'epoch': 0.99}                                                                                             
{'eval_loss': 0.9670813679695129, 'eval_auc': 0.9593949298469389, 'eval_f1_best': 0.8, 'eval_f1_threshold': 0.2398681640625, 'eval_mcc_best': 0.7893522173763263, 'eval_mcc_threshold': 0.74951171875, 'eval_num_samples': 1232, 'eval_runtime': 464.82, 'eval_samples_per_second': 2.65, 'eval_steps_per_second': 0.056, 'epoch': 1.0} 
 10%|███████████▉                                                                                                           | 689/6890 [6:41:15<58:03:34, 33.71s/it[2023-09-08 00:33:53,571] [WARNING] [stage3.py:1885:step] 1 pytorch allocator cache flushes since last step. this happens when there is high memory pressure and is detrimental to performance. if this is happening frequently consider adjusting settings to reduce memory consumption. If you are unable to make the cache flushes go away consider adding get_accelerator().empty_cache() calls in your training loop to ensure that all ranks flush their caches at the same time
{'loss': 0.7972, 'learning_rate': 9.036284470246736e-05, 'epoch': 1.0}                                                                                              
{'loss': 0.2478, 'learning_rate': 9.021770682148041e-05, 'epoch': 1.02}                                                                                             
{'loss': 0.7079, 'learning_rate': 9.007256894049347e-05, 'epoch': 1.03}                                                                                             
{'loss': 0.6803, 'learning_rate': 8.992743105950654e-05, 'epoch': 1.04}                                                                                             
{'loss': 0.3606, 'learning_rate': 8.978229317851959e-05, 'epoch': 1.06}                                                                                             
{'loss': 0.7485, 'learning_rate': 8.963715529753266e-05, 'epoch': 1.07}                                                                                             
{'loss': 0.8717, 'learning_rate': 8.949201741654572e-05, 'epoch': 1.09}                                                                                             
{'loss': 0.8356, 'learning_rate': 8.934687953555879e-05, 'epoch': 1.1}                                                                                              
{'loss': 1.345, 'learning_rate': 8.920174165457185e-05, 'epoch': 1.12}                                                                                              
100%|█████████████████████████████████████████████████████████████████████████████████████████████████████████████████████████| 1488/1488 [7:24:56<00:00, 17.94s/it]
{'test_loss': 0.09817399084568024, 'test_auc': 0.9442789131623656, 'test_f1_best': 0.43841336116910234, 'test_f1_threshold': 0.9970703125, 'test_mcc_best': 0.45029675473992603, 'test_mcc_threshold': 1.0, 'test_num_samples': 71381, 'test_runtime': 26710.8608, 'test_samples_per_second': 2.672, 'test_steps_per_second': 0.056}
[2023-09-10 20:11:52,594] [INFO] [launch.py:347:main] Process 15748 exits successfully.
[2023-09-10 20:11:56,599] [INFO] [launch.py:347:main] Process 15750 exits successfully.
[2023-09-10 20:11:56,600] [INFO] [launch.py:347:main] Process 15749 exits successfully.
[2023-09-10 20:11:56,600] [INFO] [launch.py:347:main] Process 15747 exits successfully.

(PyTorch-2.0.0) root@34229c669655:/data/chentianyu/silentVuln/LLM/starcoder/scripts# ./run_exp_16.sh 
[2023-09-14 20:14:39,279] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-14 20:14:41,797] [WARNING] [runner.py:201:fetch_hostfile] Unable to find hostfile, will proceed with training with local resources only.
[2023-09-14 20:14:41,858] [INFO] [runner.py:567:main] cmd = /home/ma-user/anaconda3/envs/PyTorch-2.0.0/bin/python -u -m deepspeed.launcher.launch --world_info=eyJsb2NhbGhvc3QiOiBbMCwgMSwgMiwgM119 --master_addr=127.0.0.1 --master_port=38622 --enable_each_rank_log=None /data/chentianyu/silentVuln/LLM/starcoder/finetune_with_trainer.py --model_path /data/qiantaotao/base_models/starcoderbase --deepspeed /data/chentianyu/silentVuln/LLM/starcoder/ds_config_zero_3.json --output_dir /efs_data/chentianyu/VulFixMiner/checkpoints/exp_16 --per_device_eval_batch_size 96 --per_device_train_batch_size 32 --num_train_epochs 10 --logging_steps 10 --gradient_checkpointing true --remove_unused_columns false --fp16 true --load_best_model_at_end true --include_inputs_for_metrics true --data_seed 42 --learning_rate 1e-4 --weight_decay 0.05 --save_strategy epoch --evaluation_strategy epoch --optim adamw_torch --data_dir /data/chentianyu/VulFixMiner/v1_dataset/v1_3 --data_split_path /data/chentianyu/VulFixMiner/v2_dataset/cross_split.json --datasets_cache_dir /data/chentianyu/VulFixMiner/cache --max_seq_length 512 --neg_ratio 10 --test_only false --diff_hunk_col commit_diff --r 16 --lora_alpha 32 --lora_dropout 0.05
[2023-09-14 20:14:43,777] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-14 20:14:45,706] [INFO] [launch.py:138:main] 0 NCCL_VERSION=2.13.4-1
[2023-09-14 20:14:45,706] [INFO] [launch.py:145:main] WORLD INFO DICT: {'localhost': [0, 1, 2, 3]}
[2023-09-14 20:14:45,706] [INFO] [launch.py:151:main] nnodes=1, num_local_procs=4, node_rank=0
[2023-09-14 20:14:45,706] [INFO] [launch.py:162:main] global_rank_mapping=defaultdict(<class 'list'>, {'localhost': [0, 1, 2, 3]})
[2023-09-14 20:14:45,706] [INFO] [launch.py:163:main] dist_world_size=4
[2023-09-14 20:14:45,707] [INFO] [launch.py:165:main] Setting CUDA_VISIBLE_DEVICES=0,1,2,3
[2023-09-14 20:14:49,544] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-14 20:14:49,693] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-14 20:14:49,694] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-14 20:14:49,702] [INFO] [real_accelerator.py:158:get_accelerator] Setting ds_accelerator to cuda (auto detect)
[2023-09-14 20:14:53,615] [INFO] [comm.py:631:init_distributed] cdb=None
[2023-09-14 20:14:53,615] [INFO] [comm.py:631:init_distributed] cdb=None
[2023-09-14 20:14:53,616] [INFO] [comm.py:662:init_distributed] Initializing TorchBackend in DeepSpeed with backend nccl
[2023-09-14 20:14:53,631] [INFO] [comm.py:631:init_distributed] cdb=None
2023-09-14 20:14:53-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 2
[2023-09-14 20:14:53,645] [INFO] [comm.py:631:init_distributed] cdb=None
2023-09-14 20:14:53-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 3
2023-09-14 20:14:54-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 1
2023-09-14 20:14:54-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:1 to store for rank: 0
2023-09-14 20:14:54-[distributed_c10d.py:466]-INFO: Rank 0: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-14 20:14:54-[distributed_c10d.py:466]-INFO: Rank 1: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-14 20:14:54-[distributed_c10d.py:466]-INFO: Rank 3: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-14 20:14:54-[distributed_c10d.py:466]-INFO: Rank 2: Completed store-based barrier for key:store_based_barrier_key:1 with 4 nodes.
2023-09-14 20:14:54-[finetune_with_trainer.py:266]-INFO: ModelArguments(model_path='/data/qiantaotao/base_models/starcoderbase')
2023-09-14 20:14:54-[finetune_with_trainer.py:267]-INFO: TrainingArguments(
_n_gpu=1,
adafactor=False,
adam_beta1=0.9,
adam_beta2=0.999,
adam_epsilon=1e-08,
auto_find_batch_size=False,
bf16=False,
bf16_full_eval=False,
data_seed=42,
dataloader_drop_last=False,
dataloader_num_workers=0,
dataloader_pin_memory=True,
ddp_backend=None,
ddp_broadcast_buffers=None,
ddp_bucket_cap_mb=None,
ddp_find_unused_parameters=None,
ddp_timeout=1800,
debug=[],
deepspeed=/data/chentianyu/silentVuln/LLM/starcoder/ds_config_zero_3.json,
disable_tqdm=False,
do_eval=True,
do_predict=False,
do_train=False,
eval_accumulation_steps=None,
eval_delay=0,
eval_steps=None,
evaluation_strategy=epoch,
fp16=True,
fp16_backend=auto,
fp16_full_eval=False,
fp16_opt_level=O1,
fsdp=[],
fsdp_config={'fsdp_min_num_params': 0, 'xla': False, 'xla_fsdp_grad_ckpt': False},
fsdp_min_num_params=0,
fsdp_transformer_layer_cls_to_wrap=None,
full_determinism=False,
gradient_accumulation_steps=1,
gradient_checkpointing=True,
greater_is_better=False,
group_by_length=False,
half_precision_backend=auto,
hub_model_id=None,
hub_private_repo=False,
hub_strategy=every_save,
hub_token=<HUB_TOKEN>,
ignore_data_skip=False,
include_inputs_for_metrics=True,
jit_mode_eval=False,
label_names=None,
label_smoothing_factor=0.0,
learning_rate=0.0001,
length_column_name=length,
load_best_model_at_end=True,
local_rank=0,
log_level=passive,
log_level_replica=warning,
log_on_each_node=True,
logging_dir=/efs_data/chentianyu/VulFixMiner/checkpoints/exp_16/runs/Sep14_20-14-53_34229c669655,
logging_first_step=False,
logging_nan_inf_filter=True,
logging_steps=10,
logging_strategy=steps,
lr_scheduler_type=linear,
max_grad_norm=1.0,
max_steps=-1,
metric_for_best_model=loss,
mp_parameters=,
no_cuda=False,
num_train_epochs=10,
optim=adamw_torch,
optim_args=None,
output_dir=/efs_data/chentianyu/VulFixMiner/checkpoints/exp_16,
overwrite_output_dir=False,
past_index=-1,
per_device_eval_batch_size=96,
per_device_train_batch_size=32,
prediction_loss_only=False,
push_to_hub=False,
push_to_hub_model_id=None,
push_to_hub_organization=None,
push_to_hub_token=<PUSH_TO_HUB_TOKEN>,
ray_scope=last,
remove_unused_columns=False,
report_to=['tensorboard'],
resume_from_checkpoint=None,
run_name=/efs_data/chentianyu/VulFixMiner/checkpoints/exp_16,
save_on_each_node=False,
save_safetensors=False,
save_steps=500,
save_strategy=epoch,
save_total_limit=None,
seed=42,
sharded_ddp=[],
skip_memory_metrics=True,
tf32=None,
torch_compile=False,
torch_compile_backend=None,
torch_compile_mode=None,
torchdynamo=None,
tpu_metrics_debug=False,
tpu_num_cores=None,
use_ipex=False,
use_legacy_prediction_loop=False,
use_mps_device=False,
warmup_ratio=0.0,
warmup_steps=0,
weight_decay=0.05,
xpu_backend=None,
)
2023-09-14 20:14:54-[finetune_with_trainer.py:268]-INFO: DataArguments(data_dir='/data/chentianyu/VulFixMiner/v1_dataset/v1_3', data_split_path='/data/chentianyu/VulFixMiner/v2_dataset/cross_split.json', datasets_cache_dir='/data/chentianyu/VulFixMiner/cache', max_seq_length=512, neg_ratio=10, test_only=False, test_checkpoint=None, diff_hunk_col='commit_diff')
2023-09-14 20:14:54-[finetune_with_trainer.py:275]-INFO: GPT2TokenizerFast(name_or_path='/data/qiantaotao/base_models/starcoderbase', vocab_size=49152, model_max_length=1000000000000000019884624838656, is_fast=True, padding_side='right', truncation_side='right', special_tokens={'bos_token': '<|endoftext|>', 'eos_token': '<|endoftext|>', 'unk_token': '<|endoftext|>', 'pad_token': '<|endoftext|>', 'additional_special_tokens': ['<|endoftext|>', '<fim_prefix>', '<fim_middle>', '<fim_suffix>', '<fim_pad>', '<filename>', '<gh_stars>', '<issue_start>', '<issue_comment>', '<issue_closed>', '<jupyter_start>', '<jupyter_text>', '<jupyter_code>', '<jupyter_output>', '<empty_output>', '<commit_before>', '<commit_msg>', '<commit_after>', '<reponame>']}, clean_up_tokenization_spaces=True)
Map (num_proc=48): 100%|███████████████████████████████████████████████████████████████████████████████████████████| 11011/11011 [00:04<00:00, 2469.82 examples/s]
Map (num_proc=48): 100%|██████████████████████████████████████████████████████████████████████████████████████████████| 1232/1232 [00:04<00:00, 271.14 examples/s]
Map (num_proc=48): 100%|███████████████████████████████████████████████████████████████████████████████████████████| 71381/71381 [00:09<00:00, 7852.56 examples/s]
2023-09-14 20:17:58-[finetune_with_trainer.py:223]-INFO: 
 *** train dataset stats ***
       msg_char_len  num_msg_tokens  diff_char_len  num_diff_tokens         label
count  11011.000000    11011.000000   11011.000000     11011.000000  11011.000000
mean      54.156026       11.959858    3006.280901       859.066025      0.090909
std       37.207057        8.318044    4919.048059      1877.047358      0.287493
min        0.000000        0.000000       0.000000         0.000000      0.000000
25%       32.000000        6.000000     771.000000       222.000000      0.000000
50%       48.000000       10.000000    1650.000000       469.000000      0.000000
75%       68.000000       16.000000    3705.500000      1041.500000      0.000000
max      760.000000      150.000000  227991.000000    141341.000000      1.000000
2023-09-14 20:17:58-[finetune_with_trainer.py:223]-INFO: 
 *** valid dataset stats ***
       msg_char_len  num_msg_tokens  diff_char_len  num_diff_tokens        label
count   1232.000000     1232.000000    1232.000000      1232.000000  1232.000000
mean      52.998377       11.797078    2902.412338       822.046266     0.090909
std       38.828394        8.367050    3745.671373      1089.890731     0.287597
min        0.000000        0.000000       0.000000         0.000000     0.000000
25%       31.000000        6.000000     757.500000       221.750000     0.000000
50%       47.000000       10.000000    1698.000000       483.000000     0.000000
75%       68.000000       15.000000    3597.000000       998.500000     0.000000
max      628.000000      108.000000   57659.000000     16322.000000     1.000000
2023-09-14 20:17:58-[finetune_with_trainer.py:223]-INFO: 
 *** test dataset stats ***
       msg_char_len  num_msg_tokens  diff_char_len  num_diff_tokens         label
count  71381.000000    71381.000000   71381.000000     71381.000000  71381.000000
mean      54.697356       11.322355    2745.403062       788.202421      0.003446
std       52.838713       37.926470    4064.556131      1266.654545      0.058604
min        0.000000        0.000000       0.000000         0.000000      0.000000
25%       34.000000        6.000000     760.000000       223.000000      0.000000
50%       48.000000       10.000000    1579.000000       455.000000      0.000000
75%       67.000000       15.000000    3476.000000       991.000000      0.000000
max     9937.000000     9913.000000  354557.000000    101220.000000      1.000000
2023-09-14 20:20:44-[finetune_with_trainer.py:285]-INFO: Loading base model
2023-09-14 20:20:44-[finetune_with_trainer.py:285]-INFO: Loading base model
2023-09-14 20:20:44-[finetune_with_trainer.py:285]-INFO: Loading base model
2023-09-14 20:20:44-[finetune_with_trainer.py:282]-INFO: DatasetDict({
    train: Dataset({
        features: ['input_ids', 'attention_mask', 'label'],
        num_rows: 11011
    })
    valid: Dataset({
        features: ['input_ids', 'attention_mask', 'label'],
        num_rows: 1232
    })
    test: Dataset({
        features: ['input_ids', 'attention_mask', 'label'],
        num_rows: 71381
    })
})
2023-09-14 20:20:44-[finetune_with_trainer.py:285]-INFO: Loading base model
[2023-09-14 20:20:57,725] [INFO] [partition_parameters.py:332:__exit__] finished initializing model - num_params = 485, num_elems = 15.52B
Loading checkpoint shards: 100%|████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [02:23<00:00, 20.54s/it]
2023-09-14 20:23:21-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Loading checkpoint shards: 100%|████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [02:23<00:00, 20.55s/it]
2023-09-14 20:23:21-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Loading checkpoint shards: 100%|████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [02:23<00:00, 20.55s/it]
2023-09-14 20:23:21-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Loading checkpoint shards: 100%|████████████████████████████████████████████████████████████████████████████████████████████████████| 7/7 [02:23<00:00, 20.56s/it]
2023-09-14 20:23:21-[finetune_with_trainer.py:296]-INFO: Initializing Lora Config 
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Detected CUDA files, patching ldflags
Emitting ninja build file /root/.cache/torch_extensions/py39_cu117/cpu_adam/build.ninja...
Building extension module cpu_adam...
Allowing ninja to set a default number of workers... (overridable by setting the environment variable MAX_JOBS=N)
ninja: no work to do.
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.040055274963379 seconds
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.0162856578826904 seconds
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
Detected CUDA files, patching ldflags
Emitting ninja build file /root/.cache/torch_extensions/py39_cu117/cpu_adam/build.ninja...
Building extension module cpu_adam...
Allowing ninja to set a default number of workers... (overridable by setting the environment variable MAX_JOBS=N)
Using /root/.cache/torch_extensions/py39_cu117 as PyTorch extensions root...
ninja: no work to do.
Loading extension module cpu_adam...
Time to load cpu_adam op: 3.130756378173828 seconds
Loading extension module cpu_adam...
Time to load cpu_adam op: 2.793856382369995 seconds
2023-09-14 20:25:44-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 1
2023-09-14 20:25:44-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 3
2023-09-14 20:25:44-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 2
2023-09-14 20:25:44-[distributed_c10d.py:432]-INFO: Added key: store_based_barrier_key:2 to store for rank: 0
2023-09-14 20:25:44-[distributed_c10d.py:466]-INFO: Rank 0: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
2023-09-14 20:25:44-[distributed_c10d.py:466]-INFO: Rank 1: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
2023-09-14 20:25:44-[distributed_c10d.py:466]-INFO: Rank 3: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
2023-09-14 20:25:44-[distributed_c10d.py:466]-INFO: Rank 2: Completed store-based barrier for key:store_based_barrier_key:2 with 4 nodes.
Parameter Offload: Total persistent parameters: 2738176 in 324 params
  0%|                                                                                                                                     | 0/870 [00:00<?, ?it/s]You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
You're using a GPT2TokenizerFast tokenizer. Please note that with a fast tokenizer, using the `__call__` method is faster than using a method to encode the text followed by a call to the `pad` method to get a padded encoding.
{'loss': 1.4437, 'learning_rate': 0.0001, 'epoch': 0.11}                                                                                                          
{'loss': 1.4736, 'learning_rate': 0.0001, 'epoch': 0.23}                                                                                                          
{'loss': 1.3972, 'learning_rate': 9.919540229885058e-05, 'epoch': 0.34}                                                                                           
{'loss': 1.2233, 'learning_rate': 9.804597701149426e-05, 'epoch': 0.46}                                                                                           
{'loss': 1.2461, 'learning_rate': 9.689655172413794e-05, 'epoch': 0.57}                                                                                           
{'loss': 1.1386, 'learning_rate': 9.574712643678161e-05, 'epoch': 0.69}                                                                                           
{'loss': 1.1468, 'learning_rate': 9.471264367816093e-05, 'epoch': 0.8}                                                                                            
{'loss': 0.9983, 'learning_rate': 9.35632183908046e-05, 'epoch': 0.92}                                                                                            
{'eval_loss': 1.0229625701904297, 'eval_auc': 0.8364596619897959, 'eval_f1_best': 0.45390070921985815, 'eval_f1_threshold': 0.64990234375, 'eval_mcc_best': 0.40121804108706693, 'eval_mcc_threshold': 0.8935546875, 'eval_num_samples': 1232, 'eval_runtime': 77.2043, 'eval_samples_per_second': 15.958, 'eval_steps_per_second': 0.052, 'epoch': 1.0}
{'loss': 0.9316, 'learning_rate': 9.241379310344827e-05, 'epoch': 1.03}                                                                                           
{'loss': 0.7435, 'learning_rate': 9.126436781609195e-05, 'epoch': 1.15}                                                                                           
{'loss': 0.5645, 'learning_rate': 9.011494252873564e-05, 'epoch': 1.26}                                                                                           
{'loss': 0.6905, 'learning_rate': 8.896551724137931e-05, 'epoch': 1.38}                                                                                           
{'loss': 0.5271, 'learning_rate': 8.7816091954023e-05, 'epoch': 1.49}                                                                                             
{'loss': 0.4326, 'learning_rate': 8.666666666666667e-05, 'epoch': 1.61}                                                                                           
{'loss': 0.1122, 'learning_rate': 7.057471264367816e-05, 'epoch': 3.22}                                                                                           
{'loss': 0.0549, 'learning_rate': 6.942528735632185e-05, 'epoch': 3.33}                                                                                           
{'loss': 0.0866, 'learning_rate': 6.827586206896552e-05, 'epoch': 3.45}                                                                                           
{'loss': 0.0675, 'learning_rate': 6.71264367816092e-05, 'epoch': 3.56}                                                                                            
{'loss': 0.094, 'learning_rate': 6.597701149425288e-05, 'epoch': 3.68}                                                                                            
{'loss': 0.0774, 'learning_rate': 6.482758620689655e-05, 'epoch': 3.79}                                                                                           
{'loss': 0.0592, 'learning_rate': 6.367816091954023e-05, 'epoch': 3.91}                                                                                           
{'eval_loss': 1.4054820537567139, 'eval_auc': 0.9534797512755102, 'eval_f1_best': 0.7837837837837838, 'eval_f1_threshold': 0.6943359375, 'eval_mcc_best': 0.7624136080920392, 'eval_mcc_threshold': 0.6943359375, 'eval_num_samples': 1232, 'eval_runtime': 75.3965, 'eval_samples_per_second': 16.34, 'eval_steps_per_second': 0.053, 'epoch': 4.0}
{'loss': 0.0434, 'learning_rate': 6.25287356321839e-05, 'epoch': 4.02}                                                                                            
{'loss': 0.0484, 'learning_rate': 6.137931034482759e-05, 'epoch': 4.14}                                                                                           
{'loss': 0.0163, 'learning_rate': 6.022988505747127e-05, 'epoch': 4.25}                                                                                           
{'loss': 0.0784, 'learning_rate': 5.908045977011495e-05, 'epoch': 4.37}                                                                                           
{'loss': 0.0286, 'learning_rate': 5.7931034482758627e-05, 'epoch': 4.48}                                                                                          
{'loss': 0.0202, 'learning_rate': 5.67816091954023e-05, 'epoch': 4.6}                                                                                             
{'loss': 0.0312, 'learning_rate': 5.5632183908045976e-05, 'epoch': 4.71}                                                                                          
{'loss': 0.0107, 'learning_rate': 5.4482758620689655e-05, 'epoch': 4.83}                                                                                          
{'loss': 0.0114, 'learning_rate': 5.333333333333333e-05, 'epoch': 4.94}                                                                                           
{'eval_loss': 1.972170114517212, 'eval_auc': 0.9480707908163264, 'eval_f1_best': 0.8, 'eval_f1_threshold': 0.94287109375, 'eval_mcc_best': 0.7936017959546404, 'eval_mcc_threshold': 0.94287109375, 'eval_num_samples': 1232, 'eval_runtime': 75.1067, 'eval_samples_per_second': 16.403, 'eval_steps_per_second': 0.053, 'epoch': 5.0}
{'loss': 0.0075, 'learning_rate': 5.218390804597701e-05, 'epoch': 5.06}                                                                                           
{'loss': 0.0149, 'learning_rate': 5.10344827586207e-05, 'epoch': 5.17}                                                                                            
{'loss': 0.0307, 'learning_rate': 4.988505747126437e-05, 'epoch': 5.29}                                                                                           
{'loss': 0.0082, 'learning_rate': 4.8735632183908047e-05, 'epoch': 5.4}                                                                                           
{'loss': 0.0093, 'learning_rate': 4.7586206896551725e-05, 'epoch': 5.52}                                                                                          
{'loss': 0.0055, 'learning_rate': 4.643678160919541e-05, 'epoch': 5.63}                                                                                           
{'loss': 0.0068, 'learning_rate': 4.528735632183908e-05, 'epoch': 5.75}                                                                                           
{'loss': 0.0092, 'learning_rate': 4.413793103448276e-05, 'epoch': 5.86}                                                                                           
{'loss': 0.0007, 'learning_rate': 4.298850574712644e-05, 'epoch': 5.98}                                                                                           
{'eval_loss': 2.5320212841033936, 'eval_auc': 0.9463408801020409, 'eval_f1_best': 0.7962085308056871, 'eval_f1_threshold': 0.64501953125, 'eval_mcc_best': 0.781928027634721, 'eval_mcc_threshold': 0.98828125, 'eval_num_samples': 1232, 'eval_runtime': 74.9489, 'eval_samples_per_second': 16.438, 'eval_steps_per_second': 0.053, 'epoch': 6.0}
{'loss': 0.006, 'learning_rate': 4.1839080459770117e-05, 'epoch': 6.09}                                                                                           
{'loss': 0.0015, 'learning_rate': 4.0689655172413795e-05, 'epoch': 6.21}                                                                                          
{'loss': 0.0002, 'learning_rate': 3.954022988505747e-05, 'epoch': 6.32}                                                                                           
{'loss': 0.0008, 'learning_rate': 3.839080459770115e-05, 'epoch': 6.44}                                                                                           
{'loss': 0.0139, 'learning_rate': 3.724137931034483e-05, 'epoch': 6.55}                                                                                           
{'loss': 0.0005, 'learning_rate': 3.609195402298851e-05, 'epoch': 6.67}                                                                                           
{'loss': 0.0056, 'learning_rate': 3.4942528735632187e-05, 'epoch': 6.78}                                                                                          
{'loss': 0.0043, 'learning_rate': 3.3793103448275865e-05, 'epoch': 6.9}                                                                                           
{'eval_loss': 2.631173849105835, 'eval_auc': 0.9450534119897959, 'eval_f1_best': 0.7980295566502463, 'eval_f1_threshold': 0.7255859375, 'eval_mcc_best': 0.7933203565141672, 'eval_mcc_threshold': 0.96533203125, 'eval_num_samples': 1232, 'eval_runtime': 74.9618, 'eval_samples_per_second': 16.435, 'eval_steps_per_second': 0.053, 'epoch': 7.0}
{'loss': 0.0257, 'learning_rate': 3.264367816091954e-05, 'epoch': 7.01}                                                                                           
{'loss': 0.0004, 'learning_rate': 3.1494252873563215e-05, 'epoch': 7.13}                                                                                          
{'loss': 0.0009, 'learning_rate': 3.0344827586206897e-05, 'epoch': 7.24}                                                                                          
{'loss': 0.0032, 'learning_rate': 2.919540229885058e-05, 'epoch': 7.36}                                                                                           
{'loss': 0.001, 'learning_rate': 2.8045977011494257e-05, 'epoch': 7.47}                                                                                           
{'loss': 0.0075, 'learning_rate': 2.689655172413793e-05, 'epoch': 7.59}                                                                                           
{'loss': 0.0002, 'learning_rate': 2.574712643678161e-05, 'epoch': 7.7}                                                                                            
{'loss': 0.0003, 'learning_rate': 2.4597701149425288e-05, 'epoch': 7.82}                                                                                          
{'loss': 0.0104, 'learning_rate': 2.3448275862068967e-05, 'epoch': 7.93}                                                                                          
{'eval_loss': 2.5418906211853027, 'eval_auc': 0.9419961734693878, 'eval_f1_best': 0.7962962962962962, 'eval_f1_threshold': 0.419921875, 'eval_mcc_best': 0.7842569299918308, 'eval_mcc_threshold': 0.94287109375, 'eval_num_samples': 1232, 'eval_runtime': 74.9543, 'eval_samples_per_second': 16.437, 'eval_steps_per_second': 0.053, 'epoch': 8.0}
{'loss': 0.0004, 'learning_rate': 2.2298850574712645e-05, 'epoch': 8.05}                                                                                          
{'loss': 0.0003, 'learning_rate': 2.1149425287356323e-05, 'epoch': 8.16}                                                                                          
{'loss': 0.0001, 'learning_rate': 2e-05, 'epoch': 8.28}                                                                                                           
{'loss': 0.0006, 'learning_rate': 1.885057471264368e-05, 'epoch': 8.39}                                                                                           
{'loss': 0.0056, 'learning_rate': 1.770114942528736e-05, 'epoch': 8.51}                                                                                           
{'loss': 0.0009, 'learning_rate': 1.6551724137931037e-05, 'epoch': 8.62}                                                                                          
{'loss': 0.0002, 'learning_rate': 1.5402298850574715e-05, 'epoch': 8.74}                                                                                          
{'loss': 0.0194, 'learning_rate': 1.4252873563218392e-05, 'epoch': 8.85}                                                                                          
{'loss': 0.0002, 'learning_rate': 1.310344827586207e-05, 'epoch': 8.97}                                                                                           
{'eval_loss': 2.5963258743286133, 'eval_auc': 0.9435586734693877, 'eval_f1_best': 0.8076923076923077, 'eval_f1_threshold': 0.75146484375, 'eval_mcc_best': 0.7928765156151899, 'eval_mcc_threshold': 0.75146484375, 'eval_num_samples': 1232, 'eval_runtime': 74.9566, 'eval_samples_per_second': 16.436, 'eval_steps_per_second': 0.053, 'epoch': 9.0}
{'loss': 0.0016, 'learning_rate': 1.1954022988505748e-05, 'epoch': 9.08}                                                                                          
{'loss': 0.0002, 'learning_rate': 1.0804597701149425e-05, 'epoch': 9.2}                                                                                           
{'loss': 0.0025, 'learning_rate': 9.655172413793103e-06, 'epoch': 9.31}                                                                                           
{'loss': 0.0001, 'learning_rate': 8.505747126436782e-06, 'epoch': 9.43}                                                                                           
{'loss': 0.0001, 'learning_rate': 7.35632183908046e-06, 'epoch': 9.54}                                                                                            
{'loss': 0.0001, 'learning_rate': 6.206896551724138e-06, 'epoch': 9.66}                                                                                           
{'loss': 0.0001, 'learning_rate': 5.057471264367817e-06, 'epoch': 9.77}                                                                                           
{'loss': 0.0046, 'learning_rate': 3.908045977011494e-06, 'epoch': 9.89}                                                                                           
{'loss': 0.0005, 'learning_rate': 2.7586206896551725e-06, 'epoch': 10.0}                                                                                          
{'eval_loss': 2.549079656600952, 'eval_auc': 0.9434550382653062, 'eval_f1_best': 0.8076923076923077, 'eval_f1_threshold': 0.7734375, 'eval_mcc_best': 0.7928765156151899, 'eval_mcc_threshold': 0.7734375, 'eval_num_samples': 1232, 'eval_runtime': 75.0573, 'eval_samples_per_second': 16.414, 'eval_steps_per_second': 0.053, 'epoch': 10.0}
{'train_runtime': 31718.2514, 'train_samples_per_second': 3.472, 'train_steps_per_second': 0.027, 'train_loss': 0.2099663090517466, 'epoch': 10.0}                
100%|█████████████████████████████████████████████████████████████████████████████████████████████████████████████████████████| 870/870 [8:48:38<00:00, 36.46s/it]
100%|███████████████████████████████████████████████████████████████████████████████████████████████████████████████████████████| 186/186 [59:33<00:00, 19.21s/it]
{'test_loss': 0.21174494922161102, 'test_auc': 0.9246713423063098, 'test_f1_best': 0.32671081677704195, 'test_f1_threshold': 0.9970703125, 'test_mcc_best': 0.3272522764656447, 'test_mcc_threshold': 0.998046875, 'test_num_samples': 71381, 'test_runtime': 3591.6963, 'test_samples_per_second': 19.874, 'test_steps_per_second': 0.052}
[2023-09-15 06:14:24,224] [INFO] [launch.py:347:main] Process 31925 exits successfully.
[2023-09-15 06:14:29,230] [INFO] [launch.py:347:main] Process 31927 exits successfully.
[2023-09-15 06:14:29,230] [INFO] [launch.py:347:main] Process 31926 exits successfully.
[2023-09-15 06:14:29,231] [INFO] [launch.py:347:main] Process 31928 exits successfully.


